Nash or Stackelberg? -- A comparative study for game-theoretic AV decision-making

This paper studies game-theoretic decision-making for autonomous vehicles (AVs). A receding horizon multi-player game is formulated to model the AV decision-making problem. Two classes of games, including Nash game and Stackelber games, are developed respectively. For each of the two games, two solution settings, including pairwise games and multi-player games, are introduced, respectively, to solve the game in multi-agent scenarios. Comparative studies are conducted via statistical simulations to gain understandings of the performance of the two classes of games and of the two solution settings, respectively. The simulations are conducted in intersection-crossing scenarios, and the game performance is quantified by three metrics: safety, travel efficiency, and computational time.

==> Conclusion.tex <==
\section{Conclusion}

This paper attempts to determine the effectiveness of Stackelberg equilibrium and Nash equilibrium by comparing them in an unsupervised intersection crossing scenario. Both best-response dynamics and potential function optimization were used to find Nash equilibrium, and both strong and weak Stackelberg games were utilized in 2-player games. Nash followers and hierarchical followers were used for 3-4-player Stackelberg games. We compared simulations where both the ego and the targets agree to play the same game against cases where the targets simply maintain a constant desired speed. 

The  crash rate of games is correlated with the games' average ego speed, but this is not a perfect measure of a game's safety. Sometimes, faster egos were safer than slower egos. Instead, the safety of a game is better measured by that game's success rate at predicting the target vehicles' behaviors. 


In each test with various amounts of players, best response dynamics was the safest decision for the ego. This algorithm is also the quickest to compute for these games with a small action space. However, this will scale poorly with larger action spaces. Best response dynamics requires that we solve an optimization problem for each agent. This leads to a small computational load when the optimization problems are simple, but a large cost when the optimization problems are difficult. 





==> Introduction.tex <==
\section{Introduction}


The decision-making algorithm of an autonomous vehicle (AV) is a critical component in broadly realizing self-driving cars. For AVs to be widely implemented, several challenges need to be addressed \cite{Gonzalez2016Review}, \cite{Kiran2022DRLSurvey}. The implemented algorithm is responsible for the safety of the AV, and that responsibility extends to any passengers or cargo present. While safety is of the utmost importance, it is also crucial for one designing a decision-making algorithm to consider the flexibility and readability of the algorithm, as well as the ability of the algorithm to scale well with increased numbers of traffic agents \cite{Wang2020DecisionReview}. It is desirable that the decision-making of an AV can be understood by an average person. It is also desirable that an algorithm is flexible enough to handle several real driving scenarios. These desires create challenges with AV decision-making. 

Game theoretical solutions have been researched as a method for controlling an AV in various traffic scenarios with multiple vehicles. Nash games \cite{9810195}, \cite{lopez_lewis_liu_wan_nageshrao_filev_2022}, are fairly simple and understandable. However, specific considerations have to be made to ensure the existence of and convergence to an optimal solution. In \cite{9810195}, an uncontrolled intersection scenario is considered. Additionally, \cite{9810195} considers mixed strategies, which are probabilistic. While mixed-strategy Nash equilibrium can solve the challenges of optimal solution existence, a definite pure-strategy is desirable. A mixed-strategy solution is going to be less likely to earn people's trust. In \cite{lopez_lewis_liu_wan_nageshrao_filev_2022}, neural networks are implemented to create a Nash Q-learning algorithm. This method does not solve a global optimal problem for all agents, which makes it more comparable to the real world and reduces the computational cost. However, care has to be taken to ensure the existence of and convergence to an optimal solution. Stackelberg games \cite{hang_lv_xing_huang_hu_2021}, \cite{Ji2021LaneMergingSF}, \cite{Ji2019StochasticStackelberg}, differ from Nash games by having a leader. The leader is the player who moves before others, which can offer an advantage for the leader over the Nash optimal solution. Unfortunately, determining who the leader is in a given traffic scenario is difficult. In \cite{Ji2021LaneMergingSF}, a Stackelberg game framework is utilized for lane-merging scenarios with many players. The authors of this study chose to utilize the lower computational cost of Stackelberg games for a more complex traffic scenario. They include an estimate of the target vehicles 'politeness' in their cost function, which allows their ego to gauge how successful it would be at changing lanes. In \cite{hang_lv_xing_huang_hu_2021}, Nash and Stackelberg games are separately combined with potential field methods and model predictive control in lane-changing and overtaking scenarios. According to this study, these two games exhibit different properties. Notably, the vehicles maintain a larger gap between themselves when using Stackelberg equilibrium than with Nash equilibrium. However, \cite{hang_lv_xing_huang_hu_2021} tests their scenarios with only one set of initial conditions.

There have been many studies that apply game-theoretic decision-making to autonomous vehicle control. However, a deep understanding of each game's characteristics and properties is lacking. This paper aims to provide some understanding by comparing the performance of Nash, Stackelberg, and potential game frameworks. This study can guide game selection to meet computational costs or to achieve the safest decision.

This paper is organized as follows. Section II formulates the generic traffic optimization problem that various game-theoretic frameworks can be applied to. Section III develops a Nash game framework and an algorithm for finding the Nash equilibrium. Section IV develops a Stackelberg game framework and an algorithm for finding the Stackelberg equilibrium. Section V provides numerical studies on the safety and computational costs of these games for two-player games. Section VI provides numerical studies on the safety and computational costs of these games with more than two players. Section VII concludes the paper.



==> IntroductionComments.tex <==
 Game theory posits that by assigning values to the states and actions of players, often with a cost or utility function, the actions of logical players can be predicted. There are three popular game models, the Nash game, the potential game, and the Stackelberg game. In Nash and potential games, players make their action decisions simultaneously. In Stackelberg games, there is a leader who acts before the other players. Each game has different solutions and methods for finding players optimal move. In this paper, various game combinations are simulated to test their safety, efficiency, and computational load.


{\color{blue}First paragraph: Decision-making for autonomous driving is critical (explain why). But it is challenging to realize (list specific challenges).

Second paragraph: To capture traffic agents' interactions, game-theoretic approaches have been developed. (List the game-theoretic decision-making papers and briefly talk about their contributions, e.g., which game is used, which scenario is considered, and what are the merits and limitations of the proposed game.)

Third paragraph: Although there are many works on game-theoretic decision-making, a deep understanding of the characteristics of each game is still lacking. This paper aims to bridge the gap by comparing the performance of various game-theoretic frameworks. This study also provides guidance on the game selection under various scenarios and/or to meet various requirements (e.g., to have the least computational cost, or to achieve the safest decision). (List specific contributions.)

Fourth paragraph: Organization of your paper. }

==> NashGames.tex <==
\section{Nash Game}
In a Nash game, it is assumed that players are equal and take simultaneous actions to obtain their lowest cost. This goal can be expressed as saying that each player wants to play their best response to each other players' actions. The best response $s_i^*$ is defined as follows:
\begin{definition}[Best Response \cite{lã_chew_soong_2016}]
An action $s_i^*$ is a best response to other players' fixed actions $s_{-i}$ if and only if
\begin{equation*}
    J_i(s_i^*,s_{-i}) \leq J_i(s_i,s_{-i}) \forall s_i \in S_i
\end{equation*}
\end{definition}

If everyone plays their best response, then no player can get a lower cost by only changing their move. This is the Nash equilibrium, which is defined here:

\begin{definition}[Nash Equilibrium \cite{lã_chew_soong_2016}]
    An action set $(s_i^*,s_{-i}^*)$ is a Nash equilibrium if and only if
    \begin{equation*}
        J_i(s_i^*,s_{-i}^*) \leq J_i(s_i,s_{-i}^*) \forall i, \forall s_i \in S_i
    \end{equation*}
\end{definition}
The Nash equilibrium is a solution to the optimal control problem identified in equation \eqref{eq:problem}. Algorithm \ref{alg:NEBRD} finds the Nash equilibrium by iteratively determining each player's best responses until no one can improve their cost by changing their move. In sequential order, each player gets to determine their best response to the other players' actions. This is repeated until no player wants to change their move. The move that has been converged to is the optimal move that the agents will take.

This algorithm has problems. Generally, a Nash game has no guarantees that best response dynamics will converge to a solution. Additionally, this algorithm can get stuck in a local minimum, thus missing out on the global optimal solution. Potential games have been identified as a type of game that can solve these problems.
\begin{algorithm}[ht]

\caption{Nash Equilibrium Best Response Dynamics}
\label{alg:NEBRD}
\begin{algorithmic}[]
 
 \Input
    \Desc{$\mathcal{G}$}{Game to solve}
  
    \EndInput
    \Output
    \Desc{$s^*$}{Nash optimal move}
    
    \EndOutput
    \end{algorithmic}
    \begin{algorithmic}[1]
    \setcounter{ALG@line}{0}
    \State \hspace*{0.02in}{\bf Procedure}
   
\State \hspace*{0.2in}{\bf For} {$i \in \mathcal{N}$} {\bf do}
\State \hspace*{0.3in}$s_i^* = 0$
\State \hspace*{0.2in}{\bf End For}
\State \hspace*{0.2in} $s^* = (s_1^*,s_2^*,...,s_N^*)$
\State \hspace*{0.2in} NECondition = 0
\State \hspace*{0.2in} {\bf While} {NECondiiton=0} {\bf do}
\State \hspace*{0.3in}$s_{prev} = s^*$
\State \hspace*{0.3in}{\bf For} {$i \in \mathcal{N}$} {\bf do}
\State \hspace*{0.4in}$s_i^* = \max_{s_i \in S_i} J_{i,tot}(s_i,s_{-i}^*)$
\State \hspace*{0.3in}{\bf  End For}
\State \hspace*{0.3in}$s^* = (s_1^*,s_2^*,...,s_N^*)$
\State \hspace*{0.3in} {\bf If} {$s^*=s_{prev}$} {\bf then}
\State \hspace*{0.4in} NECondition = 1
\State \hspace*{0.3in}{\bf  End IF}
\State \hspace*{0.2in}{\bf  End While}

 \end{algorithmic}
 
\end{algorithm}

\subsection{Finite Potential Games}
Finite potential games have been identified as a solution to the challenges faced when solving a Nash game with best response dynamics.
\begin{definition}[Finite Potential Game \cite{liu_kolmanovsky_tseng_huang_filev_girard_2023}]
    A game is a finite potential game if and only if the strategy space $S_i (i \in \mathcal{N})$ contains a finite number of elements and a potential function $P:\mathbb{S}\mapsto\mathbb{R}$ exists such that, $\forall i \in \mathcal{N}$,
    \begin{equation} 
        \begin{aligned}
             &J_i(s_i(t),s_{-i}(t))-J_i(s_i^'(t)(t),s_{-i}(t))\\
             &=P((s_i(t),s_{-i}(t))-P(s_i^'(t),s_{-i}(t)),\\
             &{\forall s_i(t),s_i^'(t) \in S_i \text{and} \forall s_{-i}(t) \in S_{-i}}
        \end{aligned}
    \end{equation}
    
\end{definition}

Any change in a player's utility caused by that player changing their action is the same as the change in the potential function. The important properties of this potential game are given in the following lemmas.

\begin{lemma}[Existence of Nash Equilibrium \cite{liu_kolmanovsky_tseng_huang_filev_girard_2023}]
If a game is a finite potential game then at least one Nash equilibrium exists.
\end{lemma}
\begin{lemma}[Equivalence of Nash Equilibrium Sets \cite{liu_kolmanovsky_tseng_huang_filev_girard_2023}]
If a game is a finite potential game with potential function $P$ then that game has the same Nash equilibriums as the identical-interest game $\bar{\mathcal{G}} = \{\mathcal{N},\mathbb{S},\{P\}_{i \in \mathcal{N}}\}$, where every players' utility is the potential function.
\label{lemma: NESet Equal}
\end{lemma}

It has been proven in \cite{liu_kolmanovsky_tseng_huang_filev_girard_2023} that if the players' cost functions have the form
\begin{equation}
    J_i(s_i,s_{-i})=J_i^{self}(s_i,s_{-i})+\sum_{j=1}^{n\neq i}J_{ij}(s_i,s_{-i})
\end{equation}
where $J_i(s_i,s_{-i})$ is a function $J_i:\mathbb{S}\mapsto\mathbb{R}$ composed of a self-interest tracker and a mutual interest tracker for each pair of agents that includes agent i,
then a potential function $P:\mathbb{S}\mapsto\mathbb{R}$ can be defined as the sum of all agents' utility.
\begin{equation}
     P(s_i,s_{-i})=\sum_{i=1}^{n}J_{i}(s_i,s_{-i})
 \end{equation}
 Additionally, this cost-function construction guarantees that algorithm \ref{alg:NEBRD} converges in a finite number of steps \cite{liu_kolmanovsky_tseng_huang_filev_girard_2023}. So by constructing a cost function in such a manner, the game is shown to have a solvable solution. However, this may be inefficient as a finite number of steps may still be long for larger games. To help this, lemma \ref{lemma: NESet Equal} suggests solving the identical-interest game $\bar{\mathcal{G}}$ instead. Since every player in $\bar{\mathcal{G}}$ has the same cost function $P$, it is much simpler to find the minimum argument $s^* \in \mathbb{S}$ of the potential function.


==> NumericalResults.tex <==

\section{Numerical Results}
\label{section: NumericalResults}
In this section, we conduct numerical studies to test the performance of the games introduced in Sections \ref{section:Nash} and \ref{section:Stackelberg}. We test the ego vehicle performance, including safety (quantified by crash rate), travel efficiency (quantified by the ego vehicle average speed), and computational cost (quantified by the average running time of one decision-making process) against various target vehicle (i..e, the vehicle that is not under our control) strategies. In Section we consider a two-vehicle intersection scenario as depicted in Figure \ref{fig:unsupervised scenario}. The performance of multi-vehicle scenarios is demonstrated in Section \ref{section:Sim4Players}, which is depicted in Figure \ref{fig:unsupervised scenario 4players}.

\begin{figure}
    \centering
    \resizebox{0.3\textwidth}{!}{\includegraphics{Figure_2Players.png}}
    \caption{An Unsupervised Intersection Scenario}
    \label{fig:unsupervised scenario}
\end{figure}

\subsection{Simulation Setup}

In the intersection-crossing scenario, we assume that all agents aim to cross the intersection safely and efficiently, i.e., tracking their own desired speeds while avoiding collisions. Motivated by this desire, we construct the cost functions  \eqref{eq:cost}. 
 \begin{equation}
     J_{i}(x(t),s(t))=\sum_{\tau=t}^{t+T-1 }Q_i(x(\tau),a(\tau)),
     \label{eq:cost}
 \end{equation}
where $Q_i(x(t),a(t))$ is described by Eq. \ref{eq:Q_i} and Eq. \ref{eq:Qij}.
\begin{equation}
    Q_i(x(t),a(t))=\frac{(v_i(t)-v_{i,d})^2}{v_{i,d}}+\sum_{j=1,j\neq i}^{N} Q_{ij}(x(t),a(t)),
    \label{eq:Q_i}
\end{equation}
\begin{dmath}
    {Q_{ij}(x(t),a(t)) = (\tanh(\beta (d_{x,c}^2-(x_i(t)-x_j(t))^2))+1)}\cdot\\{(\tanh(\beta (d_{y,c}^2-(y_i(t)-y_j(t))^2))+1)},
    \label{eq:Qij}
\end{dmath}
 where $v_{i,d}$ is player $i$'s desired speed, $d_{x,c}=d_{y,c}=6m$ is a safe distance that is slightly larger than half the width of the road, and $\beta=1000$ is a parameter used to ensure the $\tanh$ function in Eq. \eqref{eq:Qij}  only takes the values of $-1$ or $1$. Additionally, player $i$'s position at time $t$ is denoted as $(x_i(t),y_i(t))$ and player $i$'s speed at time $t$ is denoted as $v_i(t)$. The action space of each player is $\{-2,-1,0,1,2\} m/s^2$. The prediction horizon used in \eqref{eq:cost} is $4s$.

The vehicles' dynamics are described by the state space representation given in Eq. \eqref{eq:SSR} and Eq. \eqref{eq:SSR_output}. Let $x_i(t)=[z_i(t) , v_i(t)]^T$ be the state of player $i$ at time $t$, where $z_i(t)$ is the position of player $i$ along that player's direction of travel and $v_i(t)$ is player $i$'s velocity. Let the control $u_i(t) = a_i(t)$ be the acceleration of player $i$. Then the vehicle dynamics of player $i$ are described by:

\begin{equation}
    x_i(t+1)=\begin{bmatrix}
        1 & \Delta t  \\
        0 & 1
    \end{bmatrix} x_i(t) + \begin{bmatrix}
        0   \\
        \Delta t
    \end{bmatrix} u_i(t) ,
    \label{eq:SSR}
\end{equation}
\begin{equation}
    y_i(t)= \begin{bmatrix}
        1 & 0  \\
        0 & 1
    \end{bmatrix} x_i(t) ,
    \label{eq:SSR_output}
\end{equation}
 where $\Delta t=0.5s$ is the time between iterations.

To test the robustness of the ego vehicle strategies, we let the target vehicle take three different strategies:
\begin{itemize}
    \item ``Ideal'' meaning that the target vehicle also uses the outcome from the corresponding games, as the ego vehicle expected, representing ideal situations;
    \item ``Simple rules'' meaning that the target vehicle brakes at its maximum allowed deceleration $(-2m/s^2)$ to a stop if it does not have the right of way (i.e., further away from the intersection compared to the ego vehicle) and is in danger of crashing (i.e., $Q_{ij}(x(t+1),a(t))>0$, where $Q_{ij}$ is described by Eq. \ref{eq:Qij}). Otherwise, the target vehicle moves to keep its desired speed. Such a setting represents a safety- and rule- conscious vehicle, but its specific behaviors may not always be consistent with the ego vehicle expectation. 
    \item ``Constant speed'' meaning that the target vehicle simply keeps a constant speed and does not respond to the ego vehicle at all, representing a safety- and rule- agnostic vehicle. 
\end{itemize}

For ease of calculations, player strategies were limited such that there are two actions in a strategy, with each action happening for half of the time horizon. Since the strategy space in our study is relatively small, we evaluate each strategy to find the corresponding costs, and use the MATLAB function `min' \cite{MATLAB_min} to deriove the optimal strategy. The runtime of simulations is measured by MATLAB's `tic-toc' functions \cite{MATLAB_Tic,MATLAB_Toc} and simulations are performed on a desktop with an Intel Core i9-12900k processor clocked at 3200 MHz and 64 GB of RAM. One hundred games of each of these behaviors were simulated in MATLAB. The ego always has the same initial condition, while the targets' initial position along the x-axis is randomized. Target positions are randomized such that the target player is further from the intersection than the leader. Nash games are solved with best response dynamics. Both strong and weak Stackelberg games are played. In Stackelberg games, the ego is assumed to be the leader. For this simulation, both players' initial speeds are 4m/s, while their desired speed is 10m/s.

\subsection{2-Vehicle Intersection Crossing}

From Table \ref{table:5mcrash} we observe that all of these games show no crashes when both players agree to play the optimal move. When the target vehicle uses a different behavior, the Stackelberg games crash at a larger rate than in the Nash games. Perhaps oddly, the Nash equilibrium performs better against the constant-behavior target than it does against the simple-behavior target. There are two reasons for this. First, the constant-behavior target travels faster than the simple-behavior target, which causes it to be less likely to interact with the ego vehicle. Second, the simple-behavior only considers the possibility of a crash at the next time step, which is often far too late. The simple-behavior target is more likely to pose a threat to the ego playing the Nash equilibrium and is ill-equipped to stay safe. The Stackelberg games do not show this. In these games, the ego is more likely to place itself in the path of the constant-behavior target, anticipating that the target will yield. When the target does not yield, the ego in the Stackelberg game tends to brake, which causes it to both move slower and be in danger more often. 

The less than ideal behaviors lead to an increase in the average speed of the ego. However, this is not an increase in the efficiency, as the higher speeds also correlate to a decrease in safety. 

Table \ref{table:5mcrash} shows the average time in seconds to compute one optimal decision. The elapsed time to run $100$ scenarios of a given behavior was recorded using MATLAB's `tic-toc' functions \cite{MATLAB_Tic}\cite{MATLAB_Toc}. The time given is calculated by dividing the measured time by $100*50$ since there are $50$ games per scenario and $100$ scenarios. The different behaviors don't add any significant time, so each behavior's time is shown to serve as additional measurements.
Each decision accounts for $0.5s$ of real-time action. Each of these methods can compute a solution fast enough for a real version of the scenario used in this paper, which only involves two cars.Best response dynamics are shown in Table \ref{table:5mcrash} to be safer, more efficient, and easier to compute. Larger games with more players likely have different results, so we expand our simulations to include a third and fourth player in Section \ref{section:Sim4Players}.
\begin{Study}[Statistical Comparison of Nash Game and Stackleberg Game]\label{Study:NGvsSG}


\end{Study}
\begin{Study}[Comparison of Stackelberg Equilibriums]\label{Study:TwoStacks}
    The two different Stackelberg games had similar results in the statistical comparison. In the games where both players agreed, these two games had the same average ego speed of $9.14 m/s$, which indicates that they are behaving the same. It is expected that these games behave the same, as the utility function given by Eq. \eqref{eq:cost} makes it unlikely that a player can have a tie between two of their moves. The strong and weak Stackelberg games are not showing different behaviors in this test.

It is beneficial to test the differences between the two Stackelberg games. We can construct a scenario where these games behave differently. For simplicity, we restrict the actions of a player to the set $\mathcal{A}_i = \{-1,0,1\}m/s^2$ and strategies are restricted to only consist of the first action taken in a sequence, i.e $s_i \in \{[-1,-1],[0,0],[1,1]\}m/s^2$. Table \ref{table: sse v wse} illustrates a cost matrix which yields different behaviors in the strong and weak Stackelberg games. The cost function of this scenario is defined in a way such that Eq. \eqref{eq9} and Eq. \eqref{eq10} are true given the current states of players.
\begin{dmath} 
    C_{l}(s_l(t),s_f(t))=\max(\{10,(s_{l}(t)+s_f(t))*5+10\}) + 5*\text{abs}(s_l)-10,
    \label{eq9}
\end{dmath}
\begin{dmath}
    C_{f}(s_l(t),s_f(t))=\max(\{10,(s_{l}(t)+s_f(t))*5+10\}) + -5*(s_f(t)+1),
    \label{eq10}
\end{dmath}
    where the subscript $l$ denotes the leader and the subscript $f$ denotes the follower. The strong Stackelberg equilibrium is the strategy $\{0,0],[0,0]\}m/s^2$. Both of the strategies $\{[0,0],[1,1]\}m/s^2$ and $\{[-1,-1],[1,1]\}m/s^2$ are weak Stackelberg equilibriums. The leader ego selects its strategy to be $[-1,-1]m/s^2$ and assumes the target plays $[1,1]m/s^2$. The ego does not know that the target has instead opted to maintain its current speed. Figure \ref{fig: two Stackelberg algorithms} shows snapshots of this simulation at key times. Observe that the ego is much more conservative in the weak Stackelberg game than in the strong. The ego expects a more aggressive action from the target and reacts accordingly. Interestingly, this creates one of the few scenarios in which the ego crashes due to it taking the more conservative action. 
    
    While such a scenario does lead to different behaviors, it is impractical for normal use. To easily observe the differences between the strong and weak Stackelberg equilibriums, we use a special case where a reasonable cost function built out of conditional statements can be heavily simplified to the forms in Eq. \eqref{eq9} and Eq. \eqref{eq10}. Based on Table \ref{table:5mcrash}, the two Stackelberg games give the same results when utilizing the cost function described by Eq. \eqref{eq:cost}.
\begin{table}[ht!]
\begin{tabular}{|c|c|c|c|}
\hline
Leader\textbackslash{}Follower & -1     & 0       & 1       \\ \hline
-1                             & (5,10) & (5,5)   & (5,0)   \\ \hline
0                              & (0,10) & (0,5)   & (5,5)   \\ \hline
1                              & (5,10) & (10,10) & (15,10) \\ \hline
\end{tabular}
\caption{Cost matrix to compare strong and weak Stackelberg games}
\label{table: sse v wse}
\end{table}

\begin{figure*}[ht!]
\centering
    \begin{subfigure}[b]{\textwidth}
    \centering
    \resizebox{\textwidth}{!}{\includegraphics{images/SSE.png}}
    \caption{Strong Stackelberg equilibrium}
    \label{fig:sse_example}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
    \centering
    \resizebox{\textwidth}{!}{\includegraphics{images/WSE.png}}
    \caption{Weak Stackelberg equilibrium}
    \label{fig:wse_example}
    \end{subfigure}
    \caption{Different Stackelberg Equilibriums}
    \label{fig: two Stackelberg algorithms}
\end{figure*}
\end{Study}

\subsection{4-vehicle Intersection Crossing}



\section{Simulation Results: 2 Player}
\label{section:Sim2Player}
In this section, we conduct numerical studies to test the performance of the games introduced in Sections \ref{section:Nash} and \ref{section:Stackelberg}. Specifically, we consider a two-vehicle intersection scenario as depicted in Figure \ref{fig:unsupervised scenario}, and test the ego vehicle performance, including safety (quantified by crash rate), travel efficiency (quantified by the ego vehicle average speed), and computational cost (quantified by the average running time of one decision-making process) against various target vehicle (i..e, the vehicle that is not under our control) strategies. The performance of in multi-vehicle scenarios is demonstrated in Section \ref{section:Sim4Players}.

In the intersection-crossing scenario, we assume that all agents aim to cross the intersection safely and efficiently, i.e., tracking their own desired speeds while avoiding collisions. Motivated by this desire, we construct the cost functions  \eqref{eq:cost}. 
 \begin{equation}
     J_{i}(x(t),s(t))=\sum_{\tau=t}^{t+T-1 }Q_i(x(\tau),a(\tau)),
     \label{eq:cost}
 \end{equation}
where $Q_i(x(t),a(t))$ is described by Eq. \ref{eq:Q_i} and Eq. \ref{eq:Qij}.
\begin{equation}
    Q_i(x(t),a(t))=\frac{(v_i(t)-v_{i,d})^2}{v_{i,d}}+\sum_{j=1,j\neq i}^{N} Q_{ij}(x(t),a(t)),
    \label{eq:Q_i}
\end{equation}
\begin{dmath}
    {Q_{ij}(x(t),a(t)) = (\tanh(\beta (d_{x,c}^2-(x_i(t)-x_j(t))^2))+1)}\cdot\\{(\tanh(\beta (d_{y,c}^2-(y_i(t)-y_j(t))^2))+1)},
    \label{eq:Qij}
\end{dmath}
 where $v_{i,d}$ is player $i$'s desired speed, $d_{x,c}=d_{y,c}=6m$ is a safe distance that is slightly larger than half the width of the road, and $\beta=1000$ is a parameter used to ensure the $\tanh$ function in Eq. \eqref{eq:Qij}  only takes the values of $-1$ or $1$. Additionally, player $i$'s position at time $t$ is denoted as $(x_i(t),y_i(t))$ and player $i$'s speed at time $t$ is denoted as $v_i(t)$. The action space of each player is $\{-2,-1,0,1,2\} m/s^2$. The prediction horizon used in \eqref{eq:cost} is $4s$.

 

\begin{figure}
    \centering
    \resizebox{0.3\textwidth}{!}{\includegraphics{Figure_2Players.png}}
    \caption{An Unsupervised Intersection Scenario}
    \label{fig:unsupervised scenario}
\end{figure}

The vehicles' dynamics are described by the state space representation given in Eq. \eqref{eq:SSR} and Eq. \eqref{eq:SSR_output}. Let $x_i(t)=[z_i(t) , v_i(t)]^T$ be the state of player $i$ at time $t$, where $z_i(t)$ is the position of player $i$ along that player's direction of travel and $v_i(t)$ is player $i$'s velocity. Let the control $u_i(t) = a_i(t)$ be the acceleration of player $i$. Then the vehicle dynamics of player $i$ are described by:

\begin{equation}
    x_i(t+1)=\begin{bmatrix}
        1 & \Delta t  \\
        0 & 1
    \end{bmatrix} x_i(t) + \begin{bmatrix}
        0   \\
        \Delta t
    \end{bmatrix} u_i(t) ,
    \label{eq:SSR}
\end{equation}
\begin{equation}
    y_i(t)= \begin{bmatrix}
        1 & 0  \\
        0 & 1
    \end{bmatrix} x_i(t) ,
    \label{eq:SSR_output}
\end{equation}
 where $\Delta t=0.5s$ is the time between iterations. 
 
To test the robustness of the ego vehicle strategies, we let the target vehicle take three different strategies:
\begin{itemize}
    \item ``Ideal'' meaning that the target vehicle also uses the outcome from the corresponding games, as the ego vehicle expected, representing ideal situations;
    \item ``Simple rules'' meaning that the target vehicle brakes at its maximum allowed deceleration $(-2m/s^2)$ to a stop if it does not have the right of way (i.e., further away from the intersection compared to the ego vehicle) and is in danger of crashing (i.e., $Q_{ij}(x(t+1),a(t))>0$, where $Q_{ij}$ is described by Eq. \ref{eq:Qij}). Otherwise, the target vehicle moves to keep its desired speed. Such a setting represents a safety- and rule- conscious vehicle, but its specific behaviors may not always be consistent with the ego vehicle expectation. 
    \item ``Constant speed'' meaning that the target vehicle simply keeps a constant speed and does not respond to the ego vehicle at all, representing a safety- and rule- agnostic vehicle. 
\end{itemize} 
%The two players can agree to the same game or the target vehicle can maintain its desired speed, indicating a scenario where that driver is not paying attention. A simple rules-based behavior is also utilized. In this simple behavior, the target brakes to a stop if it does not have the right of way and is in danger of crashing. Otherwise, the target accelerates to its desired speed and maintains said speed. These behaviors are implemented to test the robustness of the different game solutions. The agreed behavior is the ideal case for two players. The simple rules behavior shows a target vehicle who is safety-concious but likely not ideal. The case where the target plays a constant speed represents a safety-agnostic driver, one who is not paying attention. It is rare that real drivers utilize game-theoretical solutions, and these behaviors are how we represent different degrees of idealism.

For ease of calculations, player strategies were limited such that there are two actions in a strategy, with each action happening for half of the time horizon. Since the strategy space in our study is relatively small, we evaluate each strategy to find the corresponding costs, and use the MATLAB function `min' \cite{MATLAB_min} to deriove the optimal strategy. The runtime of simulations is measured by MATLAB's `tic-toc' functions \cite{MATLAB_Tic,MATLAB_Toc} and simulations are performed on a desktop with an Intel Core i9-12900k processor clocked at 3200 MHz and 64 GB of RAM. One hundred games of each of these behaviors were simulated in MATLAB. The ego always has the same initial condition, while the targets' initial position along the x-axis is randomized. Target positions are randomized such that the target player is further from the intersection than the leader. Nash games are solved with best response dynamics. Both strong and weak Stackelberg games are played. In Stackelberg games, the ego is assumed to be the leader. For this simulation, both players' initial speeds are 4m/s, while their desired speed is 10m/s. Table \ref{table:5mcrash} shows the number of times that a crash occurred while the test distance D was less than five meters. If the two vehicles come within D meters of each other, then that game is considered a crash. 
 


\begin{table*}
\centering

\caption{Two Player Game}
\begin{tabular}{|c|ccc|ccc|ccc|}
\hline
Metric & \multicolumn{3}{c|}{Crashes per 100 Games} & \multicolumn{3}{c|}{Ave. Ego Speed (m/s)} & \multicolumn{3}{c|}{Ave. Decision Time (s)} \\ \hline
Behavior\textbackslash{}Game & \multicolumn{1}{c|}{SSE} & \multicolumn{1}{c|}{WSE} & NBR & \multicolumn{1}{c|}{SSE} & \multicolumn{1}{c|}{WSE} & NBR & \multicolumn{1}{c|}{SSE} & \multicolumn{1}{c|}{WSE} & NBR \\ \hline
Ideal & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} & 0 & \multicolumn{1}{c|}{9.14} & \multicolumn{1}{c|}{9.14} & 9.18 & \multicolumn{1}{c|}{0.0053} & \multicolumn{1}{c|}{0.0052} & 0.0006 \\ \hline
Simple Rules & \multicolumn{1}{c|}{14} & \multicolumn{1}{c|}{14} & 7 & \multicolumn{1}{c|}{9.15} & \multicolumn{1}{c|}{9.15} & 9.19 & \multicolumn{1}{c|}{0.0053} & \multicolumn{1}{c|}{0.0053} & 0.0006 \\ \hline
Constant Speed & \multicolumn{1}{c|}{15} & \multicolumn{1}{c|}{15} & 3 & \multicolumn{1}{c|}{9.18} & \multicolumn{1}{c|}{9.18} & 9.22 & \multicolumn{1}{c|}{0.0053} & \multicolumn{1}{c|}{0.0053} & 0.0006 \\ \hline

\end{tabular}
\caption*{$D<5 m, v_1(t_0) = 4 m/s = v_2(t_0), v_d = 10 m/s$}
\label{table:5mcrash}
\end{table*}

The strong and weak Stackelberg games only deviates slightly in the computational time by an insignificant amount, and the number of crashes and the average ego speed are the same. The strong and weak games can only differ if the follower has multiple best responses to the leader's actions. In this case, the distinction has no bearing on the Stackelberg solution. In Section \ref{subsec:StrongvWeakStack}, we construct a scenario that highlights the differences between the strong and weak Stackleberg equilibriums.

 
 \subsection{Two Stackelberg Equilibriums}
 \label{subsec:StrongvWeakStack}
The two different Stackelberg games had similar results in the statistical comparison. In the games where both players agreed, these two games had the same average ego speed of $9.14 m/s$, which indicates that they are behaving the same. It is expected that these games behave the same, as the utility function given by Eq. \eqref{eq:cost} makes it unlikely that a player can have a tie between two of their moves. The strong and weak Stackelberg games are not showing different behaviors in this test.

It is beneficial to test the differences between the two Stackelberg games. We can construct a scenario where these games behave differently. For simplicity, we restrict the actions of a player to the set $\mathcal{A}_i = \{-1,0,1\}m/s^2$ and strategies are restricted to only consist of the first action taken in a sequence, i.e $s_i \in \{[-1,-1],[0,0],[1,1]\}m/s^2$. Table \ref{table: sse v wse} illustrates a cost matrix which yields different behaviors in the strong and weak Stackelberg games. The cost function of this scenario is defined in a way such that Eq. \eqref{eq9} and Eq. \eqref{eq10} are true given the current states of players.
\begin{dmath} 
    C_{l}(s_l(t),s_f(t))=\max(\{10,(s_{l}(t)+s_f(t))*5+10\}) + 5*\text{abs}(s_l)-10,
    \label{eq9}
\end{dmath}
\begin{dmath}
    C_{f}(s_l(t),s_f(t))=\max(\{10,(s_{l}(t)+s_f(t))*5+10\}) + -5*(s_f(t)+1),
    \label{eq10}
\end{dmath}
    where the subscript $l$ denotes the leader and the subscript $f$ denotes the follower. The strong Stackelberg equilibrium is the strategy $\{0,0],[0,0]\}m/s^2$. Both of the strategies $\{[0,0],[1,1]\}m/s^2$ and $\{[-1,-1],[1,1]\}m/s^2$ are weak Stackelberg equilibriums. The leader ego selects its strategy to be $[-1,-1]m/s^2$ and assumes the target plays $[1,1]m/s^2$. The ego does not know that the target has instead opted to maintain its current speed. Figure \ref{fig: two Stackelberg algorithms} shows snapshots of this simulation at key times. Observe that the ego is much more conservative in the weak Stackelberg game than in the strong. The ego expects a more aggressive action from the target and reacts accordingly. Interestingly, this creates one of the few scenarios in which the ego crashes due to it taking the more conservative action. 
    
    While such a scenario does lead to different behaviors, it is impractical for normal use. To easily observe the differences between the strong and weak Stackelberg equilibriums, we use a special case where a reasonable cost function built out of conditional statements can be heavily simplified to the forms in Eq. \eqref{eq9} and Eq. \eqref{eq10}. Based on Table \ref{table:5mcrash}, the two Stackelberg games give the same results when utilizing the cost function described by Eq. \eqref{eq:cost}.
\begin{table}[ht!]
\begin{tabular}{|c|c|c|c|}
\hline
Leader\textbackslash{}Follower & -1     & 0       & 1       \\ \hline
-1                             & (5,10) & (5,5)   & (5,0)   \\ \hline
0                              & (0,10) & (0,5)   & (5,5)   \\ \hline
1                              & (5,10) & (10,10) & (15,10) \\ \hline
\end{tabular}
\caption{Cost matrix to compare strong and weak Stackelberg games}
\label{table: sse v wse}
\end{table}

\begin{figure*}[ht!]
\centering
    \begin{subfigure}[b]{\textwidth}
    \centering
    \resizebox{\textwidth}{!}{\includegraphics{images/SSE.png}}
    \caption{Strong Stackelberg equilibrium}
    \label{fig:sse_example}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
    \centering
    \resizebox{\textwidth}{!}{\includegraphics{images/WSE.png}}
    \caption{Weak Stackelberg equilibrium}
    \label{fig:wse_example}
    \end{subfigure}
    \caption{Different Stackelberg Equilibriums}
    \label{fig: two Stackelberg algorithms}
\end{figure*}
 
\subsection{Statistical Comparison}
\label{subsec:Comp2Player}

From Table \ref{table:5mcrash} we observe that all of these games show no crashes when both players agree to play the optimal move. When the target vehicle uses a different behavior, the Stackelberg games crash at a larger rate than in the Nash games. Perhaps oddly, the Nash equilibrium performs better against the constant-behavior target than it does against the simple-behavior target. There are two reasons for this. First, the constant-behavior target travels faster than the simple-behavior target, which causes it to be less likely to interact with the ego vehicle. Second, the simple-behavior only considers the possibility of a crash at the next time step, which is often far too late. The simple-behavior target is more likely to pose a threat to the ego playing the Nash equilibrum and is ill-equipped to stay safe. The Stackelberg games do not show this. In these games, the ego is more likely to place itself in the path of the constant-behavior target, anticipating that the target will yield. When the target does not yield, the ego in the Stackelberg game tends to brake, which causes it to both move slower and be in danger more often. 

The less than ideal behaviors lead to an increase in the average speed of the ego. However, this is not an increase in the efficiency, as the higher speeds also correlate to a decrease in safety. 

Table \ref{table:5mcrash} shows the average time in seconds to compute one optimal decision. The elapsed time to run $100$ scenarios of a given behavior was recorded using MATLAB's `tic-toc' functions \cite{MATLAB_Tic}\cite{MATLAB_Toc}. The time given is calculated by dividing the measured time by $100*50$ since there are $50$ games per scenario and $100$ scenarios. The different behaviors don't add any significant time, so each behavior's time is shown to serve as additional measurements.
Each decision accounts for $0.5s$ of real-time action. Each of these methods can compute a solution fast enough for a real version of the scenario used in this paper, which only involves two cars.Best response dynamics are shown in Table \ref{table:5mcrash} to be safer, more efficient, and easier to compute. Larger games with more players likely have different results, so we expand our simulations to include a third and fourth player in Section \ref{section:Sim4Players}.

\section{Simulation Results: Four Players}
\label{section:Sim4Players}
Now we repeat the game simulations with additional players. Two additional vehicles are introduced into the scenario. Figure \ref{fig:unsupervised scenario 4players} shows how the additional players are arranged. Initial conditions, cost functions, and the players' action spaces are kept the same as in Section \ref{section:Sim2Player}.

The results from the two-player simulations show that the strong and weak Stackelberg equilibriums should behave similarly. Both strong and weak games are considered in this section to validate those results. Additionally, both pairwise and many-player games are utilized.

Table \ref{table:5mcrash_4players} shows how often players crash in 4-player games with various algorithms. The behaviors are the same as in 2-player games. None of these algorithms account for the target vehicles not playing the equilibrium move. If a game is performing poorly when the targets maintain speed, it is because that game is likely to find an equilibrium that clashes with the targets' actual move. 

%With four players, crashes are observed even when players all agree to play the Stackelberg or Nash equilibrium. One might expect this behavior to be completely safe. However, the particular settings used in these simulations allow for a peculiar phenomenon which this paper refers to as brake delay. Brake delay is a scenario where the strategy at time $t$ calls for a non-negative acceleration at time $t$ and a negative acceleration at time $t+1$ and the optimal strategy at time $t+1$ is similar. For example, $s_1^*(t)=[0,-1]m/s^2$ and $s_1^*(t+1)=[0,-1]m/s^2$. Player 1's strategy includes braking, but player 1 does not actually brake at these times. The braking action is delayed until later, which is unsafe. This behavior could be controlled by better tuning the parameters in Eq. \eqref{eq:Qij}. 
%In 2-player games, we observed no crashes when players agreed on the equilibrium move. Here, however, we observe a crash in 7  games out of 100 strong and weak Stackelberg games. The ego goes faster in the Stackelberg games when compared to the 2-player games, but the ego goes slower in the Nash games. 

\begin{table*}
\centering
 \caption{Four Player Game}
\begin{tabular}{|c|ccc|ccc|ccc|}
\hline
Metric & \multicolumn{3}{c|}{Crashes per 100 Games} & \multicolumn{3}{c|}{Ave. Ego Speed (m/s)} & \multicolumn{3}{c|}{Ave. Decision Time (s)} \\ \hline
Behavior\textbackslash{}Game & \multicolumn{1}{c|}{SSE} & \multicolumn{1}{c|}{WSE} & NBR & \multicolumn{1}{c|}{SSE} & \multicolumn{1}{c|}{WSE} & NBR & \multicolumn{1}{c|}{SSE} & \multicolumn{1}{c|}{WSE} & NBR \\ \hline
Ideal & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} & 0 & \multicolumn{1}{c|}{9.24} & \multicolumn{1}{c|}{9.24} & 9.20 & \multicolumn{1}{c|}{3.6380} & \multicolumn{1}{c|}{3.2393} & 0.0015 \\ \hline
Simple Rules & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{4} & 9 & \multicolumn{1}{c|}{9.24} & \multicolumn{1}{c|}{9.24} & 9.23 & \multicolumn{1}{c|}{3.2309} & \multicolumn{1}{c|}{3.2337} & 0.0015 \\ \hline
Constant Speed & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{4} & 4 & \multicolumn{1}{c|}{9.22} & \multicolumn{1}{c|}{9.22} & 9.21 & \multicolumn{1}{c|}{3.2348} & \multicolumn{1}{c|}{3.2313} & 0.0014 \\ \hline
\end{tabular}

\caption*{$D<5m, v_i(t_0) = 4 m/s \: \forall i \in \mathcal{N}, v_d = 10 m/s$}
\label{table:5mcrash_4players}
\end{table*}

\begin{table*}
\centering
\caption{Four Players, Pairwise Games}
\begin{tabular}{|c|ccc|ccc|ccc|}
\hline
Metric & \multicolumn{3}{c|}{Crashes per 100 Games} & \multicolumn{3}{c|}{Ave. Ego Speed (m/s)} & \multicolumn{3}{c|}{Ave. Decision Time (s)} \\ \hline
Behavior\textbackslash{}Game & \multicolumn{1}{c|}{SSE} & \multicolumn{1}{c|}{WSE} & NBR & \multicolumn{1}{c|}{SSE} & \multicolumn{1}{c|}{WSE} & NBR & \multicolumn{1}{c|}{SSE} & \multicolumn{1}{c|}{WSE} & NBR \\ \hline
Ideal & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} & 0 & \multicolumn{1}{c|}{9.14} & \multicolumn{1}{c|}{9.14} & 9.10 & \multicolumn{1}{c|}{0.0157} & \multicolumn{1}{c|}{0.0156} & 0.0017 \\ \hline
Simple Rules & \multicolumn{1}{c|}{19} & \multicolumn{1}{c|}{19} & 19 & \multicolumn{1}{c|}{9.14} & \multicolumn{1}{c|}{9.14} & 9.07 & \multicolumn{1}{c|}{0.0158} & \multicolumn{1}{c|}{0.0157} & 0.0017 \\ \hline
Constant Speed & \multicolumn{1}{c|}{19} & \multicolumn{1}{c|}{19} & 4 & \multicolumn{1}{c|}{9.11} & \multicolumn{1}{c|}{9.11} & 9.02 & \multicolumn{1}{c|}{0.0158} & \multicolumn{1}{c|}{0.0156} & 0.0017 \\ \hline

\end{tabular}
\caption*{$D<5m, v_i(t_0) = 4 m/s \: \forall i \in \mathcal{N}, v_d = 10 m/s$}
\label{table:5mcrash_4players_pairwise}
\end{table*}

\begin{Remark}
    \label{remark:Remarks4Player}
For this test, all equilibriums are found using the `min' function \cite{MATLAB_min}, which is notably slow. Each loop through algorithm \ref{alg:NEBRD} requires us to calculate the utility of a minimum of $25\times n$ strategy profiles. The best response loop is guaranteed to terminate in a finite number of steps \cite{liu_kolmanovsky_tseng_huang_filev_girard_2023}, \cite{Shapley1994PotentialG}, but there is no way to determine how many iterations are required for algorithm \ref{alg:NEBRD} to converge. In this scenario, best response dynamics converged rather quickly, which is why it took the least computational time. However, suppose that each player has a large set of actions. This would be closer in comparison to actual vehicles, and such an action set would require a different code implementation to effectively find cost function minimums. Matlab's genetic algorithm function \cite{MathWorks} is utilized by \cite{liu_kolmanovsky_tseng_huang_filev_girard_2023} to calculate players optimal moves. Iteration would still be necessary to find Nash equilibrium with best response dynamics, but the computational time could be improved.
\end{Remark}

 

\subsection{Statistical Comparison}
\label{subsec:Comp4Player}
As in Section \ref{section:Sim2Player}, Tables \ref{table:5mcrash_4players} and \ref{table:5mcrash_4players_pairwise} show that players do not crash when they agree to play the same game. Other similar patterns arise. The Nash game performs worse against simple-behavior targets. The two Stackelberg games yield the same results. Interestingly, the pairwise games tend to be less safe than their multiplayer equivalents, despite having significantly slower average ego speeds with the pairwise setting. The pairwise games only capture pair interactions between the ego and one other player at a time. While these additional interactions can be computationally expensive, they are vital to completely capturing the relationships between multiple competing traffic agents.

Tables \ref{table:5mcrash_4players} and \ref{table:5mcrash_4players_pairwise} show that the multiplayer game setting is safer and more efficient than the pairwise setting. However, the computational cost of the multiplayer Stackelberg game is simply too high to be feasible without alterations.

We can compare the computational time taken to complete each type of game with the number of players increasing from two to four players.  Table \ref{table:5mcrash_4players} shows the real-time in seconds that it took to complete one decision.  As in the 2-player games, one decision gives the ego an action that it uses for $0.5$ seconds.

The algorithm used here for Stackleberg games is based on the algorithm described in \cite{Conitzer_Sandholm_2006}. This algorithm tests each of the followers' strategies to determine the best response, which is slow. However, since this is done without any optimization functions, such as MATLAB's 'ga' function \cite{MathWorks}, the best response is also calculated without these optimization tools.

\begin{Remark}
\label{remark:compTimeImportance}
    While computational time is important, each game's rate of crashes is the more distinguishing feature between different game types. There does not seem to be a correlation between the average ego speed and the crash rate. Nash best response gave faster speeds, yet consistently led to fewer crashes than in Stackelberg games. It seems that the main contributor to crashes is the target's behavior. The ego does not account for the targets' behavior to deviate from the optimal solution. This leads the ego towards confidently making the wrong assumptions about the targets, and that is dangerous. 
\end{Remark}


==> ProblemFormulation.tex <==
\section{Problem Formulation}
N traffic agents are in an unspecified traffic scenario. Let $\mathcal{N}=\{1,2,...,N\}$ be the set containing these agents. The action space for each agent is $S_i = \{s_1,s_2,...,s_m\} $, and $s_i \in \mathcal{S}_i$ are the actions that agent $i$ may take. Each agent is subject to the discrete vehicle dynamics in equation 1.


\begin{equation}
     x_i(t+\Delta t) = f_i(x_i(t),s_i(t)),
\end{equation}
where $\Delta t$ is a small increment in time, $x_i(t) \in \mathcal{X}_i$ is the state of agent i at time t, $a_i(t) \in \mathcal{A}_i$ is the action of agent i at time t. Let $\mathbb{A}$ be the Cartesian product $A_1 \times A_2 \times ... A_n$ and $(a_i,a_{-i}) \in \mathbb{S}$ be an action point, where $-i$ denotes every agent except agent i, i.e $-i=\{1,2,...,i-1,i+1,...,n\}$ We will also make use of action sequences, also called strategies, which will be denoted as $s_i=\{a_i(t),a_i(t+1),...,a_i(t+T-1) \}$. Let $S_i$ be the set of all possible strategies available to agent i. 

At time t each agent finds the action sequence $s_i(t)^*$ that minimizes their cumulative cost over the time horizon $\mathcal{T} = \{t,t+1,...,t+T-1\}$, that is 
\begin{equation}
    s_i(t)^* \in \argmin_{s_i(t) \in S_i} \sum_{\tau=t}^{t+T-1} J_i(x_i(\tau),s_i(\tau),x_{-i}(\tau),s_{-i}(\tau))
    \label{eq:problem}
\end{equation}

where $J_i(x_i(\tau),s_i(\tau),x_{-i}(\tau),s_{-i}(\tau))$ is a function $J_i:\mathbb{S}\times\mathcal{X}\mapsto\mathbb{R}$ that relates an agent's actions to a number. The challenge to this problem is that each agent has their own optimization problem to consider and each agent's actions affect the other agents' costs. Game theory is well suited to handle such a problem. This paper uses the Nash game and the Stackelberg game to solve this problem. Generally, a game consists of a set of players, a set of actions, and a set of cost functions. This can be expressed as $ \mathcal{G} = \{\mathcal{N},\mathbb{S},\{J_i\}_{i \in \mathcal{N}}\}$ such that a game $\mathcal{G}$ is a collection of the relevant information for that game. 


 
 

 
 



==> SimulationResults.tex <==
\section{Simulation Results: 2 Player}

Each player has their own objectives, which are assumed to consist of tracking a desired speed and remaining safe. 
Player i considers a utility function of the form
\begin{equation}
    J_i(s_i(t),s_{j}(t))=\frac{(|\textbf{v}_i(t)|-v_{i,d})^2}{v_{i,d}}+\sum J_{ij}
\end{equation}
\begin{dmath}
    {j_{ij} = (\tanh(\beta (d_{x,c}^2-(x_i(t)-x_j(t))^2))+1)}\cdot\\{(\tanh(\beta (d_{y,c}^2-(y_i(t)-y_j(t))^2))+1)}
\end{dmath}
 where $v_{i,d}$ is player i's desired speed, $d_{x,c}=d_{y,c}=4.5m$ is a safe distance that is slightly smaller than half the width of the road, and $\beta=1000$ is a parameter used to ensure that tanh(arg) takes the extreme values of -1 or 1. It is desired that a given action performs well for a duration, so the total utility is a summation of $J_i$ over a time horizon of $\tau=4s$.
 \begin{equation}
     J_{i,tot}(s_i,s_j)=\sum_{n=0}^{\tau/\Delta t}J_i(s_i(t),s_{j}(t))
     \label{eq:cost}
 \end{equation}

\begin{figure}
    \centering
    \resizebox{0.3\textwidth}{!}{\includegraphics{scenariofigure.png}}
    \caption{An Unsupervised Intersection Scenario}
    \label{fig:unsupervised scenario}
\end{figure}
 
 The different methods for generating an optimal move were combined so that the two players can generate their move under various behaviors. The two players can agree to the same game or the target vehicle can maintain its desired speed, indicating a scenario where that driver is not paying attention. For ease of calculations, player strategies were limited such that every action in a strategy is the same as the first action in that strategy. One thousand games of each of these behaviors were simulated in MATLAB. The ego always has the same initial condition, while the target's initial position along the x-axis is randomized. Nash games are solved with best response dynamics and with potential function optimization. Both strong and weak Stackelberg games are played. For this simulation, both players' initial speeds are 4m/s, while their desired speed is 10m/s. Table \ref{table:5mcrash} shows the number of times that a crash occurred while the test distance D was less than five meters. If the two vehicles come within D meters of each other, then that game is considered a crash.
 
\begin{table*}
\centering

\caption{Number of Crashes}
      \begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Behavior\textbackslash{}Game & Strong Stackelberg & Weak Stackelberg & Nash Best Response & Nash Potential \\ \hline
Agreed                       & 0                  & 0                & 0                  & 0              \\ \hline
Constant                     & 210                & 210              & 21                 & 130            \\ \hline
\end{tabular}
    
    \label{tab:egoF_3mcrash}
    \hfill
    \caption{Average Ego Speed}

\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Behavior\textbackslash{}Game & Strong Stackelberg & Weak Stackelberg & Nash Best Response & Nash Potential \\ \hline
Agreed                       & 8.2750             & 8.2750           & 8.3104             & 8.3501         \\ \hline
Constant                     & 8.4210             & 8.4128           & 8.2919             & 8.4494         \\ \hline
\end{tabular}

\caption*{Crashes per 1000 Games, 2 players, $D<5, v_1(t_0) = 4 m/s = v_2(t_0), v_d = 10 m/s$}
\label{table:5mcrash}
\end{table*}


 

 In simulations, crashes only occurred when the ego (player 1) was in the lead position. Best response dynamics has the fewest crashes. Both Stackelberg games had a similar number of crashes, but the weak Stackelberg game had the most crashes. When both players agree to the same game, no crashes occur. This indicates a strong experimental safety guarantee from these games. However, the assumption that both players play the same game is highly restrictive. 

 \subsection{Different Nash Solutions}
Earlier we discussed how potential function optimization gives the global optimal solution, whereas best response dynamics may get trapped in a local minimum. However, our simulations show that potential function optimization performed worse. To understand this, let us investigate an example where potential function optimization was unsafe while best response dynamics was safe. Figure \ref{fig: two nash algorithms} shows how these two different algorithms can differ under certain conditions. When the ego uses potential function optimization, it finds that it should be able to safely accelerate up to its desired speed. It expects the target to slow down a little such that both cars can safely travel at overall higher speeds. In best response dynamics, the ego slows down a bit. Table \ref{table:BestResponseDynamics} shows the values of the cost functions of the two players in the middle of the game played in figure \ref{fig: two nash algorithms}. At this time, the moves $(1,-1)$ and $(0,0)$ are the two Nash equilibriums. Adding the payoffs for both players together, we find that these moves have the same potential function value of $1.21$. This is to be expected as lemma \ref{lemma: NESet Equal} \cite{liu_kolmanovsky_tseng_huang_filev_girard_2023} states that the Nash game and the corresponding potential game have the same equilibriums. These two equilibriums corroborate the ego behaviors that can be observed in figure \ref{fig: two nash algorithms}. 

Both equilibriums should be valid control schemes for the ego. In practice, only the move $(0,0)$ is safe because it lines up with the actual behavior of the target, which is to maintain speed, rather than assume the target will rationally change its move. 

\begin{table}
\begin{tabular}{|c|c|c|c|}
\hline
Ego\textbackslash{}Target & -1            & 0         & 1             \\ \hline
-1                        & (4.015,0.935) & (4.015,0) & (4.015,0.935  \\ \hline
0                         & (1.21,0.935)  & (1.21,0)  & (1.21,0.935)  \\ \hline
1                         & (0.275,0.935) & (4.275,4) & (8.275,8.935) \\ \hline
\end{tabular}
\caption{Cost Matrix at time t=3.25s in the game played in figure \ref{fig:pfo}}
\label{table:BestResponseDynamics}
\end{table}

\begin{figure*}[ht!]
\centering
    \begin{subfigure}[b]{\textwidth}
    \centering
    \resizebox{\textwidth}{!}{\includegraphics{images/potential_figure.png}}
    \caption{Potential function optimization}
    \label{fig:pfo}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
    \centering
    \resizebox{\textwidth}{!}{\includegraphics{images/NE_figure.png}}
    \caption{Best response dynamics}
    \label{fig:brd}
    \end{subfigure}
    \caption{Different Nash Solutions}
    \label{fig: two nash algorithms}
\end{figure*}


 
 \subsection{Two Stackelberg Equilibriums}
The two different Stackelberg games had similar results. In the games where both players agreed, these two games had the same average ego speed of $8.275 m/s$, which indicates that they are behaving the same. It is expected that these games behave the same, as the utility function \eqref{eq:cost} makes it unlikely that a player can have a tie between two of their moves. 

Both games had crashes when the target vehicle had an initial x position in the range $75 m \leq x_{2}(t=0) \leq 85 m$. Since there are no differences between the conditions that lead to a crash, the seventeen additional crashes in the weak Stackelberg game can be attributed to the different occurrence rates of these conditions when generating a randomized initial condition. The strong and weak Stackelberg games are not showing different behaviors in this test.

Consider a cost function where being within a certain range of one's desired speed is worth a set amount to a player and there are a few tolerable distances between players that are allowed, although distances in a closer range are more costly than distances in a further range. With such a cost function, a cost matrix that exhibits different weak and strong Stackelberg equilibriums can be achieved. Table \ref{table: sse v wse} illustrates the cost matrix of such an example. The cost function of this is defined in a way such that \eqref{eq9} and \eqref{eq10} are true given the current states of players.
\begin{equation} 
    C_{l}=\max(10,(s_{l}+s_f)*5+10) + 5*\text{abs}(s_l)-10
    \label{eq9}
\end{equation}
\begin{equation}
    C_{f}=\max(10,(s_{l}+s_f)*5+10) + -5*(s_f+1)
    \label{eq10}
\end{equation}
    where the subscript l denotes the leader and the subscript f denotes the follower. The strong Stackelberg equilibrium is the move (0,0). Both of the moves (0,1) and (-1,1) are weak Stackelberg equilibriums. The leader ego selects its move to be $-1m/s^2$ and assumes the target will play $1m/s^2$. The ego does not know that the target has instead opted to maintain its current speed. Figure \ref{fig: two Stackelberg algorithms} shows snapshots of this simulation at key times. Observe that the ego is much more conservative in the weak Stackelberg game than in the strong. The ego expects a more aggressive action from the target and reacts accordingly. Interestingly, this creates one of the few scenarios in which the ego crashes due to it taking the more conservative action. 
    
    While such a scenario does lead to different behaviors, it is impractical for normal use. To easily observe the differences between the strong and weak Stackelberg equilibriums, we use a special case where a reasonable cost function built out of conditional statements can be heavily simplified to the forms in \eqref{eq9} and \eqref{eq10}. Based on table \ref{tab:egoF_3mcrash}, it is rare for these games to exhibit different behaviors when using the cost function \eqref{eq:cost}. The difference in the number of crashes is not significant, and it is more likely attributed to differences in the randomized initial conditions.
\begin{table}[ht!]
\begin{tabular}{|c|c|c|c|}
\hline
Leader\textbackslash{}Follower & -1     & 0       & 1       \\ \hline
-1                             & (5,10) & (5,5)   & (5,0)   \\ \hline
0                              & (0,10) & (0,5)   & (5,5)   \\ \hline
1                              & (5,10) & (10,10) & (15,10) \\ \hline
\end{tabular}
\caption{Cost matrix to compare strong and weak Stackelberg games}
\label{table: sse v wse}
\end{table}

\begin{figure*}[ht!]
\centering
    \begin{subfigure}[b]{\textwidth}
    \centering
    \resizebox{\textwidth}{!}{\includegraphics{images/SSE.png}}
    \caption{Strong Stackelberg equilibrium}
    \label{fig:sse_example}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
    \centering
    \resizebox{\textwidth}{!}{\includegraphics{images/WSE.png}}
    \caption{Weak Stackelberg equilibrium}
    \label{fig:wse_example}
    \end{subfigure}
    \caption{Different Stackelberg Equilibriums}
    \label{fig: two Stackelberg algorithms}
\end{figure*}
 
\subsection{Computational Load}
The elapsed time to run 1000 games of a given behavior was recorded using MATLAB's tic-toc functions. Of concern is the time when players agreed on the game. Other behaviors add computational load by requiring two solution computations instead of one. The total runtime of the Stackleberg games was 25.678 s, Nash best response totaled 12.4 s, and potential function optimization totaled 22.018 s. Divide these by 1000 for the average runtime of one of those games. 

\begin{equation*}
    t_{ST,ave}=\frac{25.678s}{1000} = 0.025678s
\end{equation*}

\begin{equation*}
    t_{NBR,ave}=\frac{12.4s}{1000} = 0.0124s
\end{equation*}
    
\begin{equation*}
    t_{NPF,ave}=\frac{22.018s}{1000} = 0.022018s
\end{equation*}
The real-time that each simulated game takes is 25s. Each of these methods is able to compute a solution fast enough for a real version of the scenario used in this paper, which only involves two cars. Larger games with more players will likely have different results, so we will expand our simulations to include a third player in the next section.

\section{Simulation Results: Additional Players}

Now we repeat the game simulations with additional players. Initial conditions, cost functions, and player's action spaces are kept the same as earlier. One additional vehicle is introduced into the scenario. Figure \ref{fig:unsupervised scenario 4players} shows how the additional players are arranged. 

The results from the two-player simulations show that the strong and weak Stackelberg equilibriums should behave similarly. In these many-player simulations, only the strong Stackelberg equilibrium will be used. However, we will use both algorithms \ref{alg:Nash Stackelberg Equilibrium} and \ref{alg:Hierarchy Stackelberg Equilibrium} to solve Stackelberg games with three and four players. 

Table \ref{tab:ego_5mcrash_3players} shows how often players crashed in 3-player games with various algorithms. In agreed games, each player plays their equilibrium move. In constant games, the target vehicles maintain their desired speed of $10m/s$. In 2-player games, we observed no crashes when players agreed on the equilibrium move. Here, however, we observe a crash in 115 to 130 games out of 1000. Interestingly, the average speed of the ego is slower in 3-player games than in 2-player games. The ego is recognizing these dangerous scenarios and slows down, but it realizes the danger too late and is not able to stop fast enough. These crashes do not say much about the different game models but rather speak to the importance of the control schema. These simulations limited the vehicle to discrete accelerations of $s \in \{-1,0,1\} m/s$. This simplifies calculations and reduces computational costs, but a more realistic model should allow for a larger range of accelerations. 

The hierarchical Stackelberg game resulted in the fewest crashes and the slowest average ego speed in the constant speed games. Potential function optimization had the most crashes in constant speed games, which is worse than its performance in 2-player games, relative to the other algorithms. None of these algorithms account for the target vehicles not playing the equilibrium move. If a game is performing poorly when the targets maintain speed, it is because that game is likely to find an equilibrium that clashes with the targets' actual move. This is the same observation made earlier in 2-player games when comparing the Nash best response and potential function optimization. While this seems to be a flaw of potential function optimization, this same flaw is present in all of these games, although to different degrees. 

\subsection{Computational Load}
We can compare the computational time taken to complete each type of games with the number of players increasing from two to four players. These games are Stackelberg games with hierarchical followers (SHF), Stackelberg games with Nash followers (SNF), Nash games solved with best response dynamics (NBR), and Nash games solved with potential function optimization (PFO). Table \ref{table:gameTimes} shows the real time in seconds that it took to complete one entire scenario. A complete scenario consists of 100 repeated games held 0.25s apart from each other. 

These results seem to disagree with previous studies. \cite{liu_kolmanovsky_tseng_huang_filev_girard_2023} compares the computational time of PFO and NBR and shows that PFO is faster. But the results here suggest the opposite. The algorithms that this study uses for PFO and NBR are derived from \cite{liu_kolmanovsky_tseng_huang_filev_girard_2023}. Unlike \cite{liu_kolmanovsky_tseng_huang_filev_girard_2023}, which uses Matlab's 'ga' function, this study calculates the optimal move by calculating the payoff for each possible move and selecting the move with the best payoff. This study can only get away with brute forced optimization because it uses action spaces with only three actions per player. Table \ref{table:gameTimes_ga} shows the computational time of various games when using the 'ga' function to determine optimal moves. 

\begin{table}[]
\begin{tabular}{|c|c|c|c|l|}
\hline
\#Players\textbackslash{}Game & SHF    & SNF    & NBR    & PFO    \\ \hline
2                             & 0.0172 & 0.0172 & 0.0089 & 0.0131 \\ \hline
3                             & 0.0528 & 0.0642 & 0.0133 & 0.0556 \\ \hline
4                             & 0.1643 & 0.233  & 0.0186 & 0.2261 \\ \hline
\end{tabular}
\caption{Computational time of various games in seconds}
\label{table:gameTimes}

\end{table}

\begin{table}[]
\begin{tabular}{|c|c|c|c|l|}
\hline
\#Players\textbackslash{}Game & SHF\_GA  & SNF\_GA & NBR\_GA & PFO\_GA \\ \hline
2                             & 14.081   & 7.4326  & 11.3202 & 2.531   \\ \hline
3                             & 42.284   & 12.4707 & 16.6837 & 4.1228  \\ \hline
4                             & 126.9216 & 19.4518 & 22.532  & 6.931   \\ \hline
\end{tabular}
\caption{Computational time of various games using Matlab's 'ga' in seconds}
\label{table:gameTimes_ga}
\end{table}

\subsection{Remarks}
For this test, all equilibriums are found using a brute force method, which is notably slow. This method requires us to calculate the utility of each unique strategy profile to solve the potential game, and an n-player game where players have 3 possible actions has $3^n$ unique strategy profiles. Meanwhile, each loop through algorithm \ref{alg:NEBRD} requires us to calculate the utility of a minimum of $3\times n$ strategy profiles. The best response loop is guaranteed to terminate in a finite number of steps \cite{liu_kolmanovsky_tseng_huang_filev_girard_2023}, \cite{Shapley1994PotentialG}, but there is no way to determine how many iterations will be required for algorithm \ref{alg:NEBRD} to converge. In this scenario, best response dynamics converged rather quickly, which is why it took the least computational time. However, suppose that each player has a large set of actions. This would be closer in comparison to actual vehicles, and such an action set would require a different code implementation to effectively find cost function minimums. Matlab's genetic algorithm function \cite{MathWorks} is utilized by \cite{liu_kolmanovsky_tseng_huang_filev_girard_2023} to calculate players optimal moves. Iteration would still be necessary to find Nash equilibrium with best response dynamics, but optimizing the potential function would be done with one simple use of this genetic algorithm function. 

While computational time is important, each games rate of crashes is the more distinguishing feature between different game types. There is a correlation between faster average ego speeds and more frequent crashes, but this is not perfect. Potential function optimization had the highest average ego speed in 2,3, and 4 player games while having the second highest crash rate. Hierarchical Stackelberg games had the slowest average ego speed in agreed behaviors, but it was the only game in which crashes occurred when players played the same game. Best response dynamics produced the slowest average ego speed against targets maintaining a constant speed, but only had the lowest crash rate in 2-player games. There does appear to be some truth to thinking that games with faster egos have more crashes, but this is not perfect. 

If faster ego speeds are not causing higher crash rates, can we determine what is? The insight to this question lies earlier when we discussed the two methods for finding the Nash equilibrium in a 2-player game. Remember that we found two Nash equiilibriums that both had the same potential function value, but only one was safe in practice. The safety of a strategy profile depends on the target vehicles playing their moves as predicted. If targets deviate from their expected behavior, as in the constant behavior games, then each game becomes less safe. This means that a game's crash rate is more closely tied to the success rate of that game accurately predicting target vehicles' behaviors. Slower actions do tend to perform better, but that is because equilibrium action profiles with a slower ego action are more likely to assume targets are being more aggressive. 

\begin{figure}
    \centering
    \resizebox{0.3\textwidth}{!}{\includegraphics{scenariofigure_4players.png}}
    \caption{An Unsupervised Intersection Scenario}
    \label{fig:unsupervised scenario 4players}
\end{figure}

\begin{table*}
\centering

\caption{Number of Crashes}
      \begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Behavior\textbackslash{}Game & Nash Stackelberg & Hierarchy Stackelberg & Nash Best Response & Nash Potential \\ \hline
Agreed                       & 0                  & 31               & 0                 & 0             \\ \hline
Constant                     & 358              & 65             & 90                 & 246            \\ \hline
\end{tabular}
    
    \label{tab:ego_5mcrash_3players}
    \hfill
    \caption{Average Ego Speed}

\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Behavior\textbackslash{}Game & Nash Stackelberg & Hierarchy Stackelberg & Nash Best Response & Nash Potential \\ \hline
Agreed                       & 8.2750             & 8.2213           & 8.3144             & 8.3477         \\ \hline
Constant                     & 8.4448           & 8.2875           & 8.2793             & 8.5382         \\ \hline
\end{tabular}

\caption*{Crashes per 1000 Games, 3 players, $D<5, v_i(t_0) = 4 m/s \: \forall i \in \mathcal{N}, v_d = 10 m/s$}
\label{table:5mcrash_3players}
\end{table*}


\begin{table*}
\centering

\caption{Number of Crashes}
      \begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Behavior\textbackslash{}Game & Nash Stackelberg & Hierarchy Stackelberg & Nash Best Response & Nash Potential \\ \hline
Agreed                       & 0                  & 31              & 0                 & 0             \\ \hline
Constant                     & 356               & 109             & 131                 & 271            \\ \hline
\end{tabular}
    
    \label{tab:ego_5mcrash_4players}
    \hfill
    \caption{Average Ego Speed}

\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Behavior\textbackslash{}Game & Nash Stackelberg & Hierarchy Stackelberg & Nash Best Response & Nash Potential \\ \hline
Agreed                       & 8.2750             & 8.2546           & 8.3164             & 8.3522         \\ \hline
Constant                     & 8.4499           & 8.2984           & 8.2913             & 8.5262         \\ \hline
\end{tabular}

\caption*{Crashes per 1000 Games, 4 players, $D<5, v_i(t_0) = 4 m/s \: \forall i \in \mathcal{N}, v_d = 10 m/s$}
\label{table:5mcrash_4players}
\end{table*}

==> StackelbergGames.tex <==
\section{Stackelberg Games}

Nash games rely on the assumption that every player in a game is equal. In many cases, this is a reasonable assumption. Sometimes, however, certain factors may place one player above others. In driving scenarios, for example, there are numerous 'right-of-way' rules that detail who on the road has priority over others. In such a case, it is no longer reasonable to assume that players take simultaneous actions. 

In a Stackelberg game, the leader commits to an action. The followers then play their best response to the leader's move. Stackelberg games differ from Nash games by having players move sequentially \cite{Korzhyk_Yin_Kiekintveld_Conitzer_Tambe_2011},\cite{Simaan_Cruz_1973} instead of simultaneously. While everyone is still trying to get the lowest cost, just as they do in a Nash game, this new hierarchical structure can lead to different behaviors. If a follower has multiple best responses to a given action from the leader, the follower can use the leader's cost to further evaluate their moves. This behavior necessitates two unique cases, which are called the strong and weak Stackelberg equilibriums.
\begin{definition}[Strong Stackelberg Equilibrium \cite{guo2018inducibility}] The action set $(s_L^*,s_F^*)$, where L and F refer to leader and follower, is a strong Stackelberg equilibrium if and only if
 \begin{equation*}
     (s_L^*,s_F^*) = \argmin_{s_L \in S_L} \min_{s_F \in BR(s_L)}{J_L(s_L,s_F)} 
 \end{equation*}
 where $BR(S_L)$ is the set of the followers' best responses to the leader's action $s_L$
 \label{def: SSE}
 \end{definition}
 \begin{definition}[Weak Stackelberg Equilibrium \cite{guo2018inducibility}] The action set $(s_L^*,s_F^*)$, where L and F refer to leader and follower, is a weak Stackelberg equilibrium if and only if
 \begin{equation*}
     (s_L^*,s_F^*) = \argmin_{s_L \in S_L} \max_{s_F \in BR(s_L)}{J_L(s_L,s_F)} 
 \end{equation*}
 where $BR(S_L)$ is the set of the followers' best responses to the leader's action $s_L$
 \label{def: WSE}
 \end{definition}
It is not clear at first if the ego should use the strong or the weak Stackelberg equilibrium. Several studies \cite{Wang2020DecisionReview}, \cite{Ji2019StochasticStackelberg}, \cite{Flad2017}, \cite{DBLP:journals/corr/abs-2009-06394} do not make a distinction between these two cases. Few studies make the distinction between the strong and weak Stackelberg equilibriums, as \cite{hang_lv_xing_huang_hu_2021} uses the strong and \cite{Ji2021LaneMergingSF} uses the weak. While \cite{hang_lv_xing_huang_hu_2021} and \cite{Ji2021LaneMergingSF} use one of the two Stackelberg equilibriums in their definitions, neither makes a comparison between the two types. 

When the ego is the follower, the ego should use the strong Stackelberg equilibrium. For the follower ego, the cost of the strong and weak Stackelberg moves is the same. It is reasonable then to design the ego to choose the strong Stackelberg equilibrium to benefit the leader at no harm to itself. When the ego is the leader, there is a less clear case for one move or the other. Our choice depends on our assumptions about the target vehicles, whose behaviors are outside of the ego's control. One can reasonably assume that target vehicles behave beneficially as long as this does not interfere with their motives, in which case the ego should play the strong Stackelberg equilibrium. However, one can also reasonably assume that target vehicles act as adversaries when possible, in which case the ego should play the weak Stackelberg equilibrium. Therefore, we will consider both for games when the ego is the leader.
 
To find the Stackelberg equilibrium, we determine the followers' best response to each of the leaders' possible moves. Once we have that, we can determine which of the leaders' moves has the best cost, knowing that the followers will then play their best responses. This method is akin to solving a sequential tree diagram, such as the example shown in figure \ref{fig:StackTree}. Given an action from the leader, the follower will choose their move to get their lowest cost. The leader uses this knowledge to inform and commit to their own decision. 

\begin{figure}
    \centering
    \resizebox{0.35\textwidth}{!}{\includegraphics{images/StackelbergTreeDiagram.png}}
    \caption{Tree Diagram of a Game}
    \label{fig:StackTree}
\end{figure}
\begin{algorithm}[ht]
    \caption{Strong Stackelberg Equilibrium}
    \label{alg:Strong Stackelberg Equilibrium}
    \begin{algorithmic}
    \Input
   \Desc{$\mathcal{G}$}{Game to solve}
    \EndInput
    
    \Output
    \Desc{$s_L^*$}{Optimal leader move}
    \Desc{$s_F^*$}{Optimal follower move}
    \EndOutput
    \end{algorithmic}
    \begin{algorithmic}[1]
    \State \hspace*{0.02in} {\bf Procedure}
    \State \hspace*{0.2in} Determine leader based on $x(t)$
    \State \hspace*{0.2in}{\bf For} $s_L \in S_L$ {\bf do}
    \State \hspace*{0.3in}$BR(s_L) = \argmin_{s_F \in S_F} J_F(s_L,s_F)$
    \State \hspace*{0.3in}$s_F^{*s_l} = \argmin_{s_F \in BR(s_L)} J_L(s_L,s_F) $ 
    \State \hspace*{0.2in}{\bf End For}
    \State \hspace*{0.3in}$s_L^*= \argmin_{s_L \in S_L} J_L(s_L,s_F^{*s_l})$
    \State \hspace*{0.3in}$s_F^*= \argmin_{s_F \in S_F} J_F(s_L^*,s_F)$
    
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[ht]
    \caption{Weak Stackelberg Equilibrium}
    \label{alg:Weak Stackelberg Equilibrium}
    \begin{algorithmic}
    \Input
   \Desc{$\mathcal{G}$}{Game to solve}
    \EndInput
    \Output
    \Desc{$s_L^*$}{Optimal leader move}
    \Desc{$s_F^*$}{Optimal follower move}
    \EndOutput
    \end{algorithmic}
    \begin{algorithmic}[1]
    \State \hspace*{0.02in} {\bf Procedure}
    \State \hspace*{0.2in} Determine leader based on $x(t)$
    \State \hspace*{0.2in}{\bf For} $s_L \in S_L$ {\bf do}
    \State \hspace*{0.3in}$BR(s_L) = \argmin_{s_F \in S_F} J_F(s_L,s_F)$
    \State \hspace*{0.3in}$s_F^{*s_l} = \argmax_{s_F \in BR(s_L)} J_L(s_L,s_F) $ 
    \State \hspace*{0.2in}{\bf End For}
    \State \hspace*{0.3in}$s_L^*= \argmin_{s_L \in S_L} J_L(s_L,s_F^{*s_l})$
    \State \hspace*{0.3in}$s_F^*= \argmin_{s_F \in S_F} J_F(s_L^*,s_F)$
    
    \end{algorithmic}
\end{algorithm}

Note the differences in the two algorithms for defining $s_F^{*s_l}$, which is the follower's best response to the leader's move $s_l$ after accounting for the different tie-breaking rules in the strong or weak Stackelberg games. In the strong game, the follower chooses their action from among their best responses to favor the leader. In the weak game, the follower breaks ties against the leader. This difference is only significant if the follower has multiple best responses to any of the leaders moves. Otherwise, this difference does not need to be considered. Also note that in our algorithms, we determine who is the leader based on state information. For the simulations presented in this paper, the leader is the player who is closest to the intersection at the start of the scenario.

Algorithms \ref{alg:Strong Stackelberg Equilibrium} and \ref{alg:Weak Stackelberg Equilibrium} need to be modified to use with multiple players. There are a few ways to tackle this problem. One method is to have the followers play a Nash equilibrium in response to the leader's move. Algorithm \ref{alg:Nash Stackelberg Equilibrium} describes a Stackelberg game with so-called Nash followers. 

\begin{algorithm}[ht]
    \caption{Stackelberg Equilibrium: Nash Followers}
    \label{alg:Nash Stackelberg Equilibrium}
    \begin{algorithmic}
    \Input
  \Desc{$\mathcal{G}$}{Game to solve}
    \EndInput
    \Output
    \Desc{$s_L^*$}{Optimal leader move}
    \Desc{$s_F^*$}{Optimal followers move}
    \EndOutput
    \end{algorithmic}
    \begin{algorithmic}[1]
    \State \hspace*{0.02in} {\bf Procedure}
    \State \hspace*{0.2in} Determine leader based on $x(t)$
    \State \hspace*{0.2in}{\bf For} $s_L \in S_L$ {\bf do}
    \State \hspace*{0.3in}$S_L^*=s_L$
    \State \hspace*{0.3in}$\mathbb{S}^*=S_L^* \times S_F$
    \State \hspace*{0.3in}$BR(s_L) = \text{NashEquilibrium (alg \ref{alg:NEBRD})}(\mathcal{N},x(t),f,\mathbb{S}^*,J_i)$
    \State \hspace*{0.3in}$s_F^{*s_l} = \argmin_{s_F \in BR(s_L)} J_L(s_L,s_F) $ 
    \State \hspace*{0.2in}{\bf End For}
    \State \hspace*{0.3in}$s_L^*= \argmin_{s_L \in S_L} J_L(s_L,s_F^{*s_l})$
    \State \hspace*{0.3in}$s_F^*= BR(s_L^*)$
    \end{algorithmic}
\end{algorithm}

Another option is to place the followers into a hierarchy. A follower in a hierarchical Stackelberg game plays a best response to the observed moves from players above them while considering that players below them will move after observing their move. We make use of the 'Solve' algorithm described in \cite{Conitzer_Sandholm_2006} to calculate the optimal strategy profiles. 

\begin{algorithm}[ht]
    \caption{Stackelberg Equilibrium: Hierarchy}
    \label{alg:Hierarchy Stackelberg Equilibrium}
    \begin{algorithmic}
    \Input
    \Desc{$\mathcal{G}$}{Game to solve}
    \EndInput
    \Output
    \Desc{$s_L^*$}{Optimal leader move}
    \Desc{$s_F^*$}{Optimal followers move}
    \EndOutput
    \end{algorithmic}
    \begin{algorithmic}[1]
    \State \hspace*{0.02in} {\bf Procedure}
    \State \hspace*{0.2in} Determine hierarchy based on $x(t)$
    \State \hspace*{0.2in}{\bf For} $s_L \in S_L$ {\bf do}
    \State \hspace*{0.3in}$S_L^*=s_L$
    \State \hspace*{0.3in}$\mathbb{S}^*=S_L^* \times S_F$
    \newline\Comment{Fix the current leaders action, then solve a subgame for the next player in the hierarchy}
    \State \hspace*{0.3in}$BR(s_L) = \text{Algorithm \ref{alg:Hierarchy Stackelberg Equilibrium}}(Su(\mathcal{G,s_L})$
    
    \State \hspace*{0.3in}$s_F^{*s_l} = \argmin_{s_F \in BR(s_L)} J_L(s_L,s_F) $ 
    \State \hspace*{0.2in}{\bf End For}
    \State \hspace*{0.3in}$s_L^*= \argmin_{s_L \in S_L} J_L(s_L,s_F^{*s_l})$
    \State \hspace*{0.3in}$s_F^*= BR(s_L^*)$
    
    \end{algorithmic}
\end{algorithm}

This method requires there to be a well-defined hierarchy among the players. This order of players can be determined based on the players' distance from the intersection, which is how we determine the leader role in the 2-player game. However, as players are added, there is a greater chance that two players may be at approximately the same distance from the intersection. This can create ambiguity, which may lead to unexpected and undesired consequences. To avoid this ambiguity, a hierarchy is decided when writing the simulation code and target vehicles are placed at a randomized distance from the intersection such that their order makes sense.

==> cuts.tex <==
\begin{abstract}

\end{abstract}

\begin{IEEEkeywords}

\end{IEEEkeywords}

\begin{figure}
\begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{sse_constantleader_strong.png}
    \caption{Strong Stackelberg Equilibrium} 
\end{subfigure}
   \begin{subfigure}[b]{0.45\textwidth}
     \centering
    \includegraphics[width=\textwidth]{se_constantleader_weak.png}
    \caption{Weak Stackelberg Equilibrium}
\end{subfigure}
\caption{Two Stackelberg Equilibrium Cases}
 \label{fig: strong v weak}
 \end{figure}


 This paper attempts to determine the effectiveness of Stackelberg equilibrium and Nash equilibrium in an unsupervised intersection crosssing scenario for an autonomous vehicle. Both best-response dynamics and potential function optimization were used to find Nash equilibrium, and both strong and weak Stackelberg games were utilized, so four types of games are considered. All of the games played do lead to unsafe scenarios when players have wrong information about the others. Best response dynamics has the fewest unsafe scenarios, while Stackelberg equilibrium leads to the most unsafe scenarios. Most unsafe scenarios occur when one player maintains a constant speed with no consideration of others, which should be expected. The next most dangerous category is when player 1 plays a Nash-optimal move and player 2 plays the lead Stackelberg move, or player 1 plays the lead Stackelberg move and player 2 plays the Nash-optimal move found with best response dynamics. The commonality is that someone played the leader's Stackelberg move, but the other player was playing a Nash game. With the way that the Stackelberg optimal move is determined here, it is unsafe for one player to play the leader's Stackelberg move if the other player is not playing the follower's Stackelberg move. Best response dynamics performed the best by the safety and computational efficiency tests in this study. However, best response dynamics does not scale well for games with more players. Larger action spaces, which would be more realistic, also influence computational efficiency. Potential function optimization scales nicely with increased players.
Of these popular game theoretical models for autonomous vehicle behavior, the Nash game has more promise than the Stackelberg game. Best-response dynamics performed the best in the tests in this paper, but this method may become unreliable in more complicated games. 

\begin{table*}
\centering

\caption{Number of Crashes}
      \begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Behavior\textbackslash{}Game & Nash Stackelberg & Hierarchy Stackelberg & Nash Best Response & Nash Potential \\ \hline
Agreed                       & 109                  & 103                & 96                  & 131              \\ \hline
Constant                     & 420                & 398              & 450                 & 430            \\ \hline
\end{tabular}
    
    \label{tab:egoF_3mcrash}
    \hfill
    \caption{Average Ego Speed}

\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Behavior\textbackslash{}Game & Nash Stackelberg & Hierarchy Stackelberg & Nash Best Response & Nash Potential \\ \hline
Agreed                       & 7.8             & 7.8           & 7.8             & 7.8         \\ \hline
Constant                     & 7.8            & 7.8           & 7.8             & 7.8         \\ \hline
\end{tabular}

\caption*{Crashes per 1000 Games, 4 players, $D<5, v_i(t_0) = 4 m/s \: \forall i \in \mathcal{N}, v_d = 10 m/s$}
\label{table:5mcrash}
\end{table*}

No collisions occur when the vehicles agree to play the same game. The Nash best response behavior is the safest when the target vehicle maintains a constant speed. This is due to best response dynamics tendency to select a slower, more conservative move, as evidenced by its slower average ego speed in table \ref{table:5mcrash}. The global optimal move found with potential function optimization is more likely to be unsafe than best response dynamics local optimal solution when the target is ignoring this option in favor of its own completely selfish desires. Best response dynamics performed the best by the safety and computational efficiency tests in this study. However, best response dynamics does not scale well for games with more players. Larger action spaces, which would be more realistic, also influence computational efficiency. Potential function optimization scales nicely with increased players since it can reduce multiple related optimization problems to a singular optimization problem. This benefit becomes more apparent when more vehicles are considered.



\begin{table}[]
\begin{tabular}{|c|c|c|c|l|l|l|l|l|}
\hline
\#Players\textbackslash{}Game & SHF    & SNF    & NBR    & PFO    & SHF\_GA  & SNF\_GA & NBR\_GA & PFO\_GA \\ \hline
2                             & 0.0172 & 0.0172 & 0.0089 & 0.0131 & 14.0810  & 7.4326  & 11.3202 & 2.5310  \\ \hline
3                             & 0.0528 & 0.0642 & 0.0133 & 0.0556 & 42.2840  & 12.4707 & 16.6837 & 4.1228  \\ \hline
4                             & 0.1643 & 0.233  & 0.0186 & 0.2261 & 126.9216 & 19.4518 & 22.5320 & 6.931   \\ \hline
\end{tabular}
\end{table}

This method is akin to solving a sequential tree diagram, such as the example shown in figure \ref{fig:StackTree}.

Consider a cost function where being within a certain range of one's desired speed is worth a set amount to a player and there are a few tolerable distances between players that are allowed, although distances in a closer range are more costly than distances in a further range. With such a cost function, a cost matrix that exhibits different weak and strong Stackelberg equilibriums can be achieved.

This method requires us to calculate the utility of each unique strategy profile to solve the game, and an n-player game where players have 5 possible actions has $5^n$ unique strategy profiles. Meanwhile, 




\section{Simulation Results: 2 Player}
\label{section:Sim2Player}
In this section, we conduct numerical studies to test the performance of the games introduced in Sections \ref{section:Nash} and \ref{section:Stackelberg}. Specifically, we consider a two-vehicle intersection scenario as depicted in Figure \ref{fig:unsupervised scenario}, and test the ego vehicle performance, including safety (quantified by crash rate), travel efficiency (quantified by the ego vehicle average speed), and computational cost (quantified by the average running time of one decision-making process) against various target vehicle (i..e, the vehicle that is not under our control) strategies. The performance of in multi-vehicle scenarios is demonstrated in Section \ref{section:Sim4Players}.

In the intersection-crossing scenario, we assume that all agents aim to cross the intersection safely and efficiently, i.e., tracking their own desired speeds while avoiding collisions. Motivated by this desire, we construct the cost functions  \eqref{eq:cost}. 
 \begin{equation}
     J_{i}(x(t),s(t))=\sum_{\tau=t}^{t+T-1 }Q_i(x(\tau),a(\tau)),
     \label{eq:cost}
 \end{equation}
where $Q_i(x(t),a(t))$ is described by Eq. \ref{eq:Q_i} and Eq. \ref{eq:Qij}.
\begin{equation}
    Q_i(x(t),a(t))=\frac{(v_i(t)-v_{i,d})^2}{v_{i,d}}+\sum_{j=1,j\neq i}^{N} Q_{ij}(x(t),a(t)),
    \label{eq:Q_i}
\end{equation}
\begin{dmath}
    {Q_{ij}(x(t),a(t)) = (\tanh(\beta (d_{x,c}^2-(x_i(t)-x_j(t))^2))+1)}\cdot\\{(\tanh(\beta (d_{y,c}^2-(y_i(t)-y_j(t))^2))+1)},
    \label{eq:Qij}
\end{dmath}
 where $v_{i,d}$ is player $i$'s desired speed, $d_{x,c}=d_{y,c}=6m$ is a safe distance that is slightly larger than half the width of the road, and $\beta=1000$ is a parameter used to ensure the $\tanh$ function in Eq. \eqref{eq:Qij}  only takes the values of $-1$ or $1$. Additionally, player $i$'s position at time $t$ is denoted as $(x_i(t),y_i(t))$ and player $i$'s speed at time $t$ is denoted as $v_i(t)$. The action space of each player is $\{-2,-1,0,1,2\} m/s^2$. The prediction horizon used in \eqref{eq:cost} is $4s$.

 

\begin{figure}
    \centering
    \resizebox{0.3\textwidth}{!}{\includegraphics{Figure_2Players.png}}
    \caption{An Unsupervised Intersection Scenario}
    \label{fig:unsupervised scenario}
\end{figure}

The vehicles' dynamics are described by the state space representation given in Eq. \eqref{eq:SSR} and Eq. \eqref{eq:SSR_output}. Let $x_i(t)=[z_i(t) , v_i(t)]^T$ be the state of player $i$ at time $t$, where $z_i(t)$ is the position of player $i$ along that player's direction of travel and $v_i(t)$ is player $i$'s velocity. Let the control $u_i(t) = a_i(t)$ be the acceleration of player $i$. Then the vehicle dynamics of player $i$ are described by:

\begin{equation}
    x_i(t+1)=\begin{bmatrix}
        1 & \Delta t  \\
        0 & 1
    \end{bmatrix} x_i(t) + \begin{bmatrix}
        0   \\
        \Delta t
    \end{bmatrix} u_i(t) ,
    \label{eq:SSR}
\end{equation}
\begin{equation}
    y_i(t)= \begin{bmatrix}
        1 & 0  \\
        0 & 1
    \end{bmatrix} x_i(t) ,
    \label{eq:SSR_output}
\end{equation}
 where $\Delta t=0.5s$ is the time between iterations. 
 
To test the robustness of the ego vehicle strategies, we let the target vehicle take three different strategies:
\begin{itemize}
    \item ``Ideal'' meaning that the target vehicle also uses the outcome from the corresponding games, as the ego vehicle expected, representing ideal situations;
    \item ``Simple rules'' meaning that the target vehicle brakes at its maximum allowed deceleration $(-2m/s^2)$ to a stop if it does not have the right of way (i.e., further away from the intersection compared to the ego vehicle) and is in danger of crashing (i.e., $Q_{ij}(x(t+1),a(t))>0$, where $Q_{ij}$ is described by Eq. \ref{eq:Qij}). Otherwise, the target vehicle moves to keep its desired speed. Such a setting represents a safety- and rule- conscious vehicle, but its specific behaviors may not always be consistent with the ego vehicle expectation. 
    \item ``Constant speed'' meaning that the target vehicle simply keeps a constant speed and does not respond to the ego vehicle at all, representing a safety- and rule- agnostic vehicle. 
\end{itemize} 
%The two players can agree to the same game or the target vehicle can maintain its desired speed, indicating a scenario where that driver is not paying attention. A simple rules-based behavior is also utilized. In this simple behavior, the target brakes to a stop if it does not have the right of way and is in danger of crashing. Otherwise, the target accelerates to its desired speed and maintains said speed. These behaviors are implemented to test the robustness of the different game solutions. The agreed behavior is the ideal case for two players. The simple rules behavior shows a target vehicle who is safety-concious but likely not ideal. The case where the target plays a constant speed represents a safety-agnostic driver, one who is not paying attention. It is rare that real drivers utilize game-theoretical solutions, and these behaviors are how we represent different degrees of idealism.

For ease of calculations, player strategies were limited such that there are two actions in a strategy, with each action happening for half of the time horizon. Since the strategy space in our study is relatively small, we evaluate each strategy to find the corresponding costs, and use the MATLAB function `min' \cite{MATLAB_min} to deriove the optimal strategy. The runtime of simulations is measured by MATLAB's `tic-toc' functions \cite{MATLAB_Tic,MATLAB_Toc} and simulations are performed on a desktop with an Intel Core i9-12900k processor clocked at 3200 MHz and 64 GB of RAM. One hundred games of each of these behaviors were simulated in MATLAB. The ego always has the same initial condition, while the targets' initial position along the x-axis is randomized. Target positions are randomized such that the target player is further from the intersection than the leader. Nash games are solved with best response dynamics. Both strong and weak Stackelberg games are played. In Stackelberg games, the ego is assumed to be the leader. For this simulation, both players' initial speeds are 4m/s, while their desired speed is 10m/s. Table \ref{table:5mcrash} shows the number of times that a crash occurred while the test distance D was less than five meters. If the two vehicles come within D meters of each other, then that game is considered a crash. 
 


\begin{table*}
\centering

\caption{Two Player Game}
\begin{tabular}{|c|ccc|ccc|ccc|}
\hline
Metric & \multicolumn{3}{c|}{Crashes per 100 Games} & \multicolumn{3}{c|}{Ave. Ego Speed (m/s)} & \multicolumn{3}{c|}{Ave. Decision Time (s)} \\ \hline
Behavior\textbackslash{}Game & \multicolumn{1}{c|}{SSE} & \multicolumn{1}{c|}{WSE} & NBR & \multicolumn{1}{c|}{SSE} & \multicolumn{1}{c|}{WSE} & NBR & \multicolumn{1}{c|}{SSE} & \multicolumn{1}{c|}{WSE} & NBR \\ \hline
Ideal & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} & 0 & \multicolumn{1}{c|}{9.14} & \multicolumn{1}{c|}{9.14} & 9.18 & \multicolumn{1}{c|}{0.0053} & \multicolumn{1}{c|}{0.0052} & 0.0006 \\ \hline
Simple Rules & \multicolumn{1}{c|}{14} & \multicolumn{1}{c|}{14} & 7 & \multicolumn{1}{c|}{9.15} & \multicolumn{1}{c|}{9.15} & 9.19 & \multicolumn{1}{c|}{0.0053} & \multicolumn{1}{c|}{0.0053} & 0.0006 \\ \hline
Constant Speed & \multicolumn{1}{c|}{15} & \multicolumn{1}{c|}{15} & 3 & \multicolumn{1}{c|}{9.18} & \multicolumn{1}{c|}{9.18} & 9.22 & \multicolumn{1}{c|}{0.0053} & \multicolumn{1}{c|}{0.0053} & 0.0006 \\ \hline

\end{tabular}
\caption*{$D<5 m, v_1(t_0) = 4 m/s = v_2(t_0), v_d = 10 m/s$}
\label{table:5mcrash}
\end{table*}

The strong and weak Stackelberg games only deviates slightly in the computational time by an insignificant amount, and the number of crashes and the average ego speed are the same. The strong and weak games can only differ if the follower has multiple best responses to the leader's actions. In this case, the distinction has no bearing on the Stackelberg solution. In Section \ref{subsec:StrongvWeakStack}, we construct a scenario that highlights the differences between the strong and weak Stackleberg equilibriums.

 
 \subsection{Two Stackelberg Equilibriums}
 \label{subsec:StrongvWeakStack}
The two different Stackelberg games had similar results. In the games where both players agreed, these two games had the same average ego speed of $9.14 m/s$, which indicates that they are behaving the same. It is expected that these games behave the same, as the utility function given by Eq. \eqref{eq:cost} makes it unlikely that a player can have a tie between two of their moves. The strong and weak Stackelberg games are not showing different behaviors in this test.

It is beneficial to test the differences between the two Stackelberg games. We can construct a scenario where these games behave differently. For simplicity, we restrict the actions of a player to the set $\mathcal{A}_i = \{-1,0,1\}m/s^2$ and strategies are restricted to only consist of the first action taken in a sequence, i.e $s_i \in \{[-1,-1],[0,0],[1,1]\}m/s^2$. Table \ref{table: sse v wse} illustrates a cost matrix which yields different behaviors in the strong and weak Stackelberg games. The cost function of this scenario is defined in a way such that Eq. \eqref{eq9} and Eq. \eqref{eq10} are true given the current states of players.
\begin{dmath} 
    C_{l}(s_l(t),s_f(t))=\max(\{10,(s_{l}(t)+s_f(t))*5+10\}) + 5*\text{abs}(s_l)-10,
    \label{eq9}
\end{dmath}
\begin{dmath}
    C_{f}(s_l(t),s_f(t))=\max(\{10,(s_{l}(t)+s_f(t))*5+10\}) + -5*(s_f(t)+1),
    \label{eq10}
\end{dmath}
    where the subscript $l$ denotes the leader and the subscript $f$ denotes the follower. The strong Stackelberg equilibrium is the strategy $\{0,0],[0,0]\}m/s^2$. Both of the strategies $\{[0,0],[1,1]\}m/s^2$ and $\{[-1,-1],[1,1]\}m/s^2$ are weak Stackelberg equilibriums. The leader ego selects its strategy to be $[-1,-1]m/s^2$ and assumes the target plays $[1,1]m/s^2$. The ego does not know that the target has instead opted to maintain its current speed. Figure \ref{fig: two Stackelberg algorithms} shows snapshots of this simulation at key times. Observe that the ego is much more conservative in the weak Stackelberg game than in the strong. The ego expects a more aggressive action from the target and reacts accordingly. Interestingly, this creates one of the few scenarios in which the ego crashes due to it taking the more conservative action. 
    
    While such a scenario does lead to different behaviors, it is impractical for normal use. To easily observe the differences between the strong and weak Stackelberg equilibriums, we use a special case where a reasonable cost function built out of conditional statements can be heavily simplified to the forms in Eq. \eqref{eq9} and Eq. \eqref{eq10}. Based on Table \ref{table:5mcrash}, the two Stackelberg games give the same results when utilizing the cost function described by Eq. \eqref{eq:cost}.
\begin{table}[ht!]
\begin{tabular}{|c|c|c|c|}
\hline
Leader\textbackslash{}Follower & -1     & 0       & 1       \\ \hline
-1                             & (5,10) & (5,5)   & (5,0)   \\ \hline
0                              & (0,10) & (0,5)   & (5,5)   \\ \hline
1                              & (5,10) & (10,10) & (15,10) \\ \hline
\end{tabular}
\caption{Cost matrix to compare strong and weak Stackelberg games}
\label{table: sse v wse}
\end{table}

\begin{figure*}[ht!]
\centering
    \begin{subfigure}[b]{\textwidth}
    \centering
    \resizebox{\textwidth}{!}{\includegraphics{images/SSE.png}}
    \caption{Strong Stackelberg equilibrium}
    \label{fig:sse_example}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
    \centering
    \resizebox{\textwidth}{!}{\includegraphics{images/WSE.png}}
    \caption{Weak Stackelberg equilibrium}
    \label{fig:wse_example}
    \end{subfigure}
    \caption{Different Stackelberg Equilibriums}
    \label{fig: two Stackelberg algorithms}
\end{figure*}
 
\subsection{Statistical Comparison}
\label{subsec:Comp2Player}

From Table \ref{table:5mcrash} we observe that all of these games show no crashes when both players agree to play the optimal move. When the target vehicle uses a different behavior, the Stackelberg games crash at a larger rate than in the Nash games. Perhaps oddly, the Nash equilibrium performs better against the constant-behavior target than it does against the simple-behavior target. There are two reasons for this. First, the constant-behavior target travels faster than the simple-behavior target, which causes it to be less likely to interact with the ego vehicle. Second, the simple-behavior only considers the possibility of a crash at the next time step, which is often far too late. The simple-behavior target is more likely to pose a threat to the ego playing the Nash equilibrum and is ill-equipped to stay safe. The Stackelberg games do not show this. In these games, the ego is more likely to place itself in the path of the constant-behavior target, anticipating that the target will yield. When the target does not yield, the ego in the Stackelberg game tends to brake, which causes it to both move slower and be in danger more often. 

The less than ideal behaviors lead to an increase in the average speed of the ego. However, this is not an increase in the efficiency, as the higher speeds also correlate to a decrease in safety. 

Table \ref{table:5mcrash} shows the average time in seconds to compute one optimal decision. The elapsed time to run $100$ scenarios of a given behavior was recorded using MATLAB's `tic-toc' functions \cite{MATLAB_Tic}\cite{MATLAB_Toc}. The time given is calculated by dividing the measured time by $100*50$ since there are $50$ games per scenario and $100$ scenarios. The different behaviors don't add any significant time, so each behavior's time is shown to serve as additional measurements.
Each decision accounts for $0.5s$ of real-time action. Each of these methods can compute a solution fast enough for a real version of the scenario used in this paper, which only involves two cars.Best response dynamics are shown in Table \ref{table:5mcrash} to be safer, more efficient, and easier to compute. Larger games with more players likely have different results, so we expand our simulations to include a third and fourth player in Section \ref{section:Sim4Players}.

\section{Simulation Results: Four Players}
\label{section:Sim4Players}
Now we repeat the game simulations with additional players. Two additional vehicles are introduced into the scenario. Figure \ref{fig:unsupervised scenario 4players} shows how the additional players are arranged. Initial conditions, cost functions, and the players' action spaces are kept the same as in Section \ref{section:Sim2Player}.

The results from the two-player simulations show that the strong and weak Stackelberg equilibriums should behave similarly. Both strong and weak games are considered in this section to validate those results. Additionally, both pairwise and many-player games are utilized.

Table \ref{table:5mcrash_4players} shows how often players crash in 4-player games with various algorithms. The behaviors are the same as in 2-player games. None of these algorithms account for the target vehicles not playing the equilibrium move. If a game is performing poorly when the targets maintain speed, it is because that game is likely to find an equilibrium that clashes with the targets' actual move. 

%With four players, crashes are observed even when players all agree to play the Stackelberg or Nash equilibrium. One might expect this behavior to be completely safe. However, the particular settings used in these simulations allow for a peculiar phenomenon which this paper refers to as brake delay. Brake delay is a scenario where the strategy at time $t$ calls for a non-negative acceleration at time $t$ and a negative acceleration at time $t+1$ and the optimal strategy at time $t+1$ is similar. For example, $s_1^*(t)=[0,-1]m/s^2$ and $s_1^*(t+1)=[0,-1]m/s^2$. Player 1's strategy includes braking, but player 1 does not actually brake at these times. The braking action is delayed until later, which is unsafe. This behavior could be controlled by better tuning the parameters in Eq. \eqref{eq:Qij}. 
%In 2-player games, we observed no crashes when players agreed on the equilibrium move. Here, however, we observe a crash in 7  games out of 100 strong and weak Stackelberg games. The ego goes faster in the Stackelberg games when compared to the 2-player games, but the ego goes slower in the Nash games. 

\begin{table*}
\centering
 \caption{Four Player Game}
\begin{tabular}{|c|ccc|ccc|ccc|}
\hline
Metric & \multicolumn{3}{c|}{Crashes per 100 Games} & \multicolumn{3}{c|}{Ave. Ego Speed (m/s)} & \multicolumn{3}{c|}{Ave. Decision Time (s)} \\ \hline
Behavior\textbackslash{}Game & \multicolumn{1}{c|}{SSE} & \multicolumn{1}{c|}{WSE} & NBR & \multicolumn{1}{c|}{SSE} & \multicolumn{1}{c|}{WSE} & NBR & \multicolumn{1}{c|}{SSE} & \multicolumn{1}{c|}{WSE} & NBR \\ \hline
Ideal & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} & 0 & \multicolumn{1}{c|}{9.24} & \multicolumn{1}{c|}{9.24} & 9.20 & \multicolumn{1}{c|}{3.6380} & \multicolumn{1}{c|}{3.2393} & 0.0015 \\ \hline
Simple Rules & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{4} & 9 & \multicolumn{1}{c|}{9.24} & \multicolumn{1}{c|}{9.24} & 9.23 & \multicolumn{1}{c|}{3.2309} & \multicolumn{1}{c|}{3.2337} & 0.0015 \\ \hline
Constant Speed & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{4} & 4 & \multicolumn{1}{c|}{9.22} & \multicolumn{1}{c|}{9.22} & 9.21 & \multicolumn{1}{c|}{3.2348} & \multicolumn{1}{c|}{3.2313} & 0.0014 \\ \hline
\end{tabular}

\caption*{$D<5m, v_i(t_0) = 4 m/s \: \forall i \in \mathcal{N}, v_d = 10 m/s$}
\label{table:5mcrash_4players}
\end{table*}

\begin{table*}
\centering
\caption{Four Players, Pairwise Games}
\begin{tabular}{|c|ccc|ccc|ccc|}
\hline
Metric & \multicolumn{3}{c|}{Crashes per 100 Games} & \multicolumn{3}{c|}{Ave. Ego Speed (m/s)} & \multicolumn{3}{c|}{Ave. Decision Time (s)} \\ \hline
Behavior\textbackslash{}Game & \multicolumn{1}{c|}{SSE} & \multicolumn{1}{c|}{WSE} & NBR & \multicolumn{1}{c|}{SSE} & \multicolumn{1}{c|}{WSE} & NBR & \multicolumn{1}{c|}{SSE} & \multicolumn{1}{c|}{WSE} & NBR \\ \hline
Ideal & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} & 0 & \multicolumn{1}{c|}{9.14} & \multicolumn{1}{c|}{9.14} & 9.10 & \multicolumn{1}{c|}{0.0157} & \multicolumn{1}{c|}{0.0156} & 0.0017 \\ \hline
Simple Rules & \multicolumn{1}{c|}{19} & \multicolumn{1}{c|}{19} & 19 & \multicolumn{1}{c|}{9.14} & \multicolumn{1}{c|}{9.14} & 9.07 & \multicolumn{1}{c|}{0.0158} & \multicolumn{1}{c|}{0.0157} & 0.0017 \\ \hline
Constant Speed & \multicolumn{1}{c|}{19} & \multicolumn{1}{c|}{19} & 4 & \multicolumn{1}{c|}{9.11} & \multicolumn{1}{c|}{9.11} & 9.02 & \multicolumn{1}{c|}{0.0158} & \multicolumn{1}{c|}{0.0156} & 0.0017 \\ \hline

\end{tabular}
\caption*{$D<5m, v_i(t_0) = 4 m/s \: \forall i \in \mathcal{N}, v_d = 10 m/s$}
\label{table:5mcrash_4players_pairwise}
\end{table*}

\begin{Remark}
    \label{remark:Remarks4Player}
For this test, all equilibriums are found using the `min' function \cite{MATLAB_min}, which is notably slow. Each loop through algorithm \ref{alg:NEBRD} requires us to calculate the utility of a minimum of $25\times n$ strategy profiles. The best response loop is guaranteed to terminate in a finite number of steps \cite{liu_kolmanovsky_tseng_huang_filev_girard_2023}, \cite{Shapley1994PotentialG}, but there is no way to determine how many iterations are required for algorithm \ref{alg:NEBRD} to converge. In this scenario, best response dynamics converged rather quickly, which is why it took the least computational time. However, suppose that each player has a large set of actions. This would be closer in comparison to actual vehicles, and such an action set would require a different code implementation to effectively find cost function minimums. Matlab's genetic algorithm function \cite{MathWorks} is utilized by \cite{liu_kolmanovsky_tseng_huang_filev_girard_2023} to calculate players optimal moves. Iteration would still be necessary to find Nash equilibrium with best response dynamics, but the computational time could be improved.
\end{Remark}

 

\subsection{Statistical Comparison}
\label{subsec:Comp4Player}
As in Section \ref{section:Sim2Player}, Tables \ref{table:5mcrash_4players} and \ref{table:5mcrash_4players_pairwise} show that players do not crash when they agree to play the same game. Other similar patterns arise. The Nash game performs worse against simple-behavior targets. The two Stackelberg games yield the same results. Interestingly, the pairwise games tend to be less safe than their multiplayer equivalents, despite having significantly slower average ego speeds with the pairwise setting. The pairwise games only capture pair interactions between the ego and one other player at a time. While these additional interactions can be computationally expensive, they are vital to completely capturing the relationships between multiple competing traffic agents.

Tables \ref{table:5mcrash_4players} and \ref{table:5mcrash_4players_pairwise} show that the multiplayer game setting is safer and more efficient than the pairwise setting. However, the computational cost of the multiplayer Stackelberg game is simply too high to be feasible without alterations.

We can compare the computational time taken to complete each type of game with the number of players increasing from two to four players.  Table \ref{table:5mcrash_4players} shows the real-time in seconds that it took to complete one decision.  As in the 2-player games, one decision gives the ego an action that it uses for $0.5$ seconds.

The algorithm used here for Stackleberg games is based on the algorithm described in \cite{Conitzer_Sandholm_2006}. This algorithm tests each of the followers' strategies to determine the best response, which is slow. However, since this is done without any optimization functions, such as MATLAB's 'ga' function \cite{MathWorks}, the best response is also calculated without these optimization tools.

\begin{Remark}
\label{remark:compTimeImportance}
    While computational time is important, each game's rate of crashes is the more distinguishing feature between different game types. There does not seem to be a correlation between the average ego speed and the crash rate. Nash best response gave faster speeds, yet consistently led to fewer crashes than in Stackelberg games. It seems that the main contributor to crashes is the target's behavior. The ego does not account for the targets' behavior to deviate from the optimal solution. This leads the ego towards confidently making the wrong assumptions about the targets, and that is dangerous. 
\end{Remark}



 





\begin{figure}
    \centering
    \resizebox{0.3\textwidth}{!}{\includegraphics{Figure_4Players.png}}
    \caption{An Unsupervised Intersection Scenario}
    \label{fig:unsupervised scenario 4players}
\end{figure}
